Calabi-Yau threefolds in positive characteristic

In this note, an overview of Calabi-Yau varieties in positive characteristic is presented. Although Calabi-Yau varieties in characteristic zero are unobstructed, there are examples of Calabi-Yau threefolds in positive characteristic which cannot be lifted to characteristic zero, although one-dimensional and two-dimensional Calabi-Yau varieties, i.e., elliptic curves and K3 surfaces, are all liftable to characteristic zero. In this respect, Calabi-Yau threefolds in positive characteristic are interesting in view of deformation theory and they are still very mysterious.

==> Name_Surname.tex <==
\begin{document} 
\selectlanguage{english}
\title{Lecture Title}
\author{Name Surname}
\affilation{
	Title. Name Surname \\
	\url{email@address} \\
	Faculty \\
	University
}
\smallFoot
\maketitle
\begin{abstract}
	Put your abstract here.
\end{abstract}
%
% ============ PUT CONTENT BETWEEN THESE MARKERS ============
%

\section{Information}\label{sec}

The contents of one paragraph.
You should rename this file and remove the example content.
To show what longer paragraphs look like, we
added this sentence.

One should use an empty line in the source code to separate consectutive
paragraphs.
This is what a reference to a section looks like: \ref{sec}.

\section{Environments defined in the preamble}

\subsection{Theorem Styled}

\begin{theorem}[Name of the theorem - this is optional and works in all these
environments]\label{thm}
	Theorem contents.
	\begin{proof}
		Proof of the theorem. One can use the \verb+proof+ environment everywhere,
		not only within environments like \verb+theorem+, \verb+algorithm+ etc.
	\end{proof}
\end{theorem}

This is what a reference to a theorem looks like: \ref{thm}.

\begin{algorithm}
	Description of the algorithm.
\end{algorithm}

\begin{conjecture}
	Conjecture contents.
\end{conjecture}

\begin{corollary}
	Corollary contents.
\end{corollary}

\begin{exercise}
	Exercise contents.
\end{exercise}

\begin{fact}
	Fact contents.
\end{fact}

\begin{hypothesis}
	Hypothesis contents.
\end{hypothesis}

\begin{lemma}
	Lemma contents.
\end{lemma}

\begin{observation}
	Observation contents.
\end{observation}

\begin{problem}
	Problem contents.
\end{problem}

\begin{property}
	Property contents.
\end{property}

\begin{proposition}
	Proposition contents.
\end{proposition}

\begin{statement}
	Statement contents.
\end{statement}

\begin{sublemma}
	Sublemma contents.
\end{sublemma}

\subsection{Definition Styled}

\begin{definition}
	Definition contents.
\end{definition}

\begin{assumption}
	Assumption contents.
\end{assumption}

\begin{example}
	Example contents.
\end{example}

\subsection{Other}

\begin{remark}
	Remark contents.
\end{remark}

\section{Frequently used environments}

\subsection{Mathematical environments}

We use the \verb+equation+ environment for numbered mathematical
expressions, for example equations (\ref{equa}):
\begin{equation}\label{equa}
	a^2 + b^2 = c^2.
\end{equation}

For non-numbered, but indented expressions we use \verb+displaymath+ or
\verb+equation*+:
\begin{equation*}
	2 + 2 = 5.
\end{equation*}

One should not use double dollars (\verb+$$+) for getting the above effect,
for it isn't consistent with the standards and might stop working without
warning. However, using single dollars for inline expressions is alright: $e^{i\pi}+1=0$. 

It is also bad to use \verb+eqnarray+. Instead one should use \verb+align+
and similiar environments when they are needed. For more information on
mathematical environments see
\url{ftp://ftp.ams.org/ams/doc/amsmath/amsldoc.pdf}.

\subsection{Floating environments}

\begin{table}[h!t]
	\centering
	\begin{tabular}{|l|l|}
		\hline
			pro & per \\
		\hline
			tab & le \\
		\hline
	\end{tabular}
	\caption{Proper table}
	\label{tab:proper}
\end{table}

\begin{figure}[h!b]
	\centering
	\includegraphics{Name_Surname-pic1.png}
	\caption{Not funny at all}
	\label{fig:smieszne}
\end{figure}

\FloatBarrier

References to a table \ref{tab:proper} and a picture
\ref{fig:smieszne}.

\subsection{Other environments}

\begin{enumerate}
	\item\label{point} Point.
	\item Following point.
\end{enumerate}

\begin{itemize}
	\item Point.
	\item Other point.
\end{itemize}

Reference to a point \ref{point}.

\section{References to numbered elements}

Using commands \verb+\label{+\textit{somelabel}\verb+}+ and
\verb+\ref{+\textit{somelabel}\verb+}+ one can refer to sections, subsections
etc., theorems, numbered equations, tables, pictures and numbered points.
One can use any string of alphanumerical characters and punctuation as
\textit{somelabel}.

Examples can be found in the text above.

\section{Literature}

One should use the command \verb+thebibliography+ for creating literature.

It is advised that only those works which are directly referenced in the text
be placed in the bibliography. The references should be placed in the order in
which they are placed in the text.

This is what references to the literature can look like: \cite{book},
\cite{book,article-printed,article-online},
\cite[Th.~1]{article-online}.

\begin{thebibliography}{99}
	\bibitem{book} Surname, Initials. \emph{Title of Book}. Place of
	publication: Publisher, year of publication.
	
	\bibitem{article-printed} Surname, Initials. "Title of
	Article." \emph{Title of Journal} VolumeNumber.IssueNumber (Year of
	publication): Page number(s).
	
	\bibitem{article-online} Surname, Initials. "Title of Article" \emph{Title of Web Page/Magazine/Encyclopedia/Project}.
	Date of article. Last accessed on Date. \url{URL}.
\end{thebibliography}

%
% ============ PUT CONTENT BETWEEN THESE MARKERS ============
%
\bigFoot
\end{document}


==> preamble.tex <==

\setlength{\textheight}{600pt}
\setlength{\textwidth}{470pt}
\setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt}
\setlength{\footskip}{40pt}
\setlength{\headheight}{15pt}

\newcommand{\bigFoot}{ \setlength{\textheight}{550pt} }
\newcommand{\smallFoot}{ \setlength{\textheight}{600pt} }

\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amsopn}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{color}
\usepackage{enumerate}
\usepackage{epsfig}
\usepackage{url}
\usepackage{fancyhdr}
\usepackage{titling}
\usepackage{longtable}
\usepackage{pstricks}
\usepackage{multido}
\usepackage{placeins}
\usepackage{clrscode}

%Abstrakt
\setlength{\abstitleskip}{-\parindent}
\setlength{\absleftindent}{0pt}
\setlength{\absrightindent}{0pt}
\abslabeldelim{.}
%Asbtrakt

%Tytul
\renewcommand{\importtitlefont}{\begin{flushleft}\LARGE\bfseries}
\renewcommand{\postimporttitle}{\par\end{flushleft}\vskip 5pt}
%Tytul

%Autor
\renewcommand{\importauthorfont}{\begin{flushleft}\large\bfseries}
\renewcommand{\postimportauthor}{\par\end{flushleft}\vskip 50pt}
%Autor

%Afiliacja
\def\theaffilation {}
\newcommand{\affilation}[1]{\def \theaffilation {#1}}
%Afiliacja

%Wyglad stron
\fancypagestyle{myheadings}{%
	\fancyhf{}%
	\fancyhead[R]{\thepage}%
	\fancyhead[L]{XVI International Workshop for Young Mathematicians}%
}
\fancypagestyle{myplain}{%
	\fancyhf{}%
	\fancyhead[R]{\thepage}%
	\fancyhead[L]{XVI International Workshop for Young Mathematicians}%
	\fancyfoot[L]{\small{\theaffilation}}%
	\renewcommand{\footrulewidth}{0.4pt}
}
\fancypagestyle{plain}{%
	\fancyhf{}%
}
\pagestyle{fancy}
	\fancyhead{}
	\fancyhead[LO]{\thetitle}
	\fancyhead[RE]{\theauthor}
	\fancyfoot{}
	\fancyhead[RO,LE]{\thepage}
	\renewcommand{\headrulewidth}{0.4pt}
	\renewcommand{\footrulewidth}{0pt}
%Wyglad stron

%Kropki
\makeatletter
\renewcommand\@seccntformat[1]{\csname the#1\endcsname.\quad}
\makeatother
%Kropki

%Przypisy
\let\oldfootnote\footnote
\renewcommand\footnote[1]{\oldfootnote{\ #1}}
%Przypisy

%Polskie spacje (przed poczatkiem zdania NIE robi sie wiekszej!)
\frenchspacing
%Polskie spacje

\theoremstyle{plain}
\newtheorem{theorem}{\iflanguage{english}{Theorem}{Twierdzenie}}
\newtheorem{algorithm}[theorem]{\iflanguage{english}{Algorithm}{Algorytm}}
\newtheorem{conjecture}[theorem]{\iflanguage{english}{Conjecture}{Przypuszczenie}}
\newtheorem{corollary}[theorem]{\iflanguage{english}{Corollary}{Wniosek}}
\newtheorem{exercise}[theorem]{\iflanguage{english}{Exercise}{\'Cwiczenie}}
\newtheorem{fact}[theorem]{\iflanguage{english}{Fact}{Fakt}}
\newtheorem{hypothesis}[theorem]{\iflanguage{english}{Hypothesis}{Hipoteza}}
\newtheorem{lemma}[theorem]{\iflanguage{english}{Lemma}{Lemat}}
\newtheorem{observation}[theorem]{\iflanguage{english}{Observation}{Obserwacja}}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{property}[theorem]{\iflanguage{english}{Property}{W{\l}asno\'s\'c}}
\newtheorem{proposition}[theorem]{\iflanguage{english}{Proposition}{Propozycja}}
\newtheorem{question}[theorem]{Question}
\newtheorem{statement}[theorem]{\iflanguage{english}{Statement}{Stwierdzenie}}
\newtheorem{sublemma}[theorem]{\iflanguage{english}{Sublemma}{Podlemat}}


\theoremstyle{definition}
\newtheorem{assumption}[theorem]{\iflanguage{english}{Assumption}{Za{\l}o{\.z}enie}}
\newtheorem{definition}[theorem]{\iflanguage{english}{Def\mbox{}inition}{Def\mbox{}inicja}}
\newtheorem{example}[theorem]{\iflanguage{english}{Example}{Przyk{\l}ad}}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{\iflanguage{english}{Remark}{Uwaga}}

\let\Omega\varOmega
\let\Phi\varPhi
\let\Psi\varPsi
\let\Gamma\varGamma
\let\Delta\varDelta
\let\Lambda\varLambda
\let\Theta\varTheta
\let\kappa\varkappa
\let\epsilon\varepsilon
\let\phi\varphi


\endinput


==> preambleArciv.tex <==

\setlength{\textheight}{600pt}
\setlength{\textwidth}{470pt}
\setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt}
\setlength{\footskip}{40pt}
\setlength{\headheight}{15pt}

\newcommand{\bigFoot}{ \setlength{\textheight}{550pt} }
\newcommand{\smallFoot}{ \setlength{\textheight}{600pt} }

\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amsopn}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{color}
\usepackage{enumerate}
\usepackage{epsfig}
\usepackage{url}
\usepackage{fancyhdr}
\usepackage{titling}
\usepackage{longtable}
\usepackage{pstricks}
\usepackage{multido}
\usepackage{placeins}
\usepackage{clrscode}

%Abstrakt
\setlength{\abstitleskip}{-\parindent}
\setlength{\absleftindent}{0pt}
\setlength{\absrightindent}{0pt}
\abslabeldelim{.}
%Asbtrakt

%Tytul
\renewcommand{\importtitlefont}{\begin{flushleft}\LARGE\bfseries}
\renewcommand{\postimporttitle}{\par\end{flushleft}\vskip 5pt}
%Tytul

%Autor
\renewcommand{\importauthorfont}{\begin{flushleft}\large\bfseries}
\renewcommand{\postimportauthor}{\par\end{flushleft}\vskip 50pt}
%Autor

%Afiliacja
\def\theaffilation {}
\newcommand{\affilation}[1]{\def \theaffilation {#1}}
%Afiliacja

%Wyglad stron
\fancypagestyle{myheadings}{%
	\fancyhf{}%
	\fancyhead[R]{\thepage}%
%\fancyhead[L]{XVI International Workshop for Young Mathematicians}%
}
\fancypagestyle{myplain}{%
	\fancyhf{}%
	\fancyhead[R]{\thepage}%
%	\fancyhead[L]{XVI International Workshop for Young Mathematicians}%
	\fancyfoot[L]{\small{\theaffilation}}%
	\renewcommand{\footrulewidth}{0.4pt}
}
\fancypagestyle{plain}{%
	\fancyhf{}%
}
\pagestyle{fancy}
	\fancyhead{}
	\fancyhead[LO]{\thetitle}
	\fancyhead[RE]{\theauthor}
	\fancyfoot{}
	\fancyhead[RO,LE]{\thepage}
	\renewcommand{\headrulewidth}{0.4pt}
	\renewcommand{\footrulewidth}{0pt}
%Wyglad stron

%Kropki
\makeatletter
\renewcommand\@seccntformat[1]{\csname the#1\endcsname.\quad}
\makeatother
%Kropki

%Przypisy
\let\oldfootnote\footnote
\renewcommand\footnote[1]{\oldfootnote{\ #1}}
%Przypisy

%Polskie spacje (przed poczatkiem zdania NIE robi sie wiekszej!)
\frenchspacing
%Polskie spacje

\theoremstyle{plain}
\newtheorem{theorem}{\iflanguage{english}{Theorem}{Twierdzenie}}
\newtheorem{algorithm}[theorem]{\iflanguage{english}{Algorithm}{Algorytm}}
\newtheorem{conjecture}[theorem]{\iflanguage{english}{Conjecture}{Przypuszczenie}}
\newtheorem{corollary}[theorem]{\iflanguage{english}{Corollary}{Wniosek}}
\newtheorem{exercise}[theorem]{\iflanguage{english}{Exercise}{\'Cwiczenie}}
\newtheorem{fact}[theorem]{\iflanguage{english}{Fact}{Fakt}}
\newtheorem{hypothesis}[theorem]{\iflanguage{english}{Hypothesis}{Hipoteza}}
\newtheorem{lemma}[theorem]{\iflanguage{english}{Lemma}{Lemat}}
\newtheorem{observation}[theorem]{\iflanguage{english}{Observation}{Obserwacja}}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{property}[theorem]{\iflanguage{english}{Property}{W{\l}asno\'s\'c}}
\newtheorem{proposition}[theorem]{\iflanguage{english}{Proposition}{Propozycja}}
\newtheorem{question}[theorem]{Question}
\newtheorem{statement}[theorem]{\iflanguage{english}{Statement}{Stwierdzenie}}
\newtheorem{sublemma}[theorem]{\iflanguage{english}{Sublemma}{Podlemat}}


\theoremstyle{definition}
\newtheorem{assumption}[theorem]{\iflanguage{english}{Assumption}{Za{\l}o{\.z}enie}}
\newtheorem{definition}[theorem]{\iflanguage{english}{Def\mbox{}inition}{Def\mbox{}inicja}}
\newtheorem{example}[theorem]{\iflanguage{english}{Example}{Przyk{\l}ad}}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{\iflanguage{english}{Remark}{Uwaga}}

\let\Omega\varOmega
\let\Phi\varPhi
\let\Psi\varPsi
\let\Gamma\varGamma
\let\Delta\varDelta
\let\Lambda\varLambda
\let\Theta\varTheta
\let\kappa\varkappa
\let\epsilon\varepsilon
\let\phi\varphi


\endinput


==> pstricks.tex <==
%% pstricks.tex
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2000-2003 by Denis Girou.
%% Copyright 2004-2006 Herbert Voss
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2003/12/01 or later.
%
% This work has the LPPL maintenance status "maintained".
% 
% This Current Maintainer of this work is Herbert Voss
%
% This work consists of the file pstricks.tex, PostScript macros 
% for Generic TeX.
% See the PSTricks User's Guide for description.
% This uses the header file `pstricks.pro'.
%
\def\fileversion{1.15}
\def\filedate{2006/12/22}
%
\csname PSTricksLoaded\endcsname
\let\PSTricksLoaded\endinput
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\expandafter\ifx\csname @latexerr\endcsname\relax
\long\def\@ifundefined#1#2#3{\expandafter\ifx\csname
  #1\endcsname\relax#2\else#3\fi}
\def\@namedef#1{\expandafter\def\csname #1\endcsname}
\def\@nameuse#1{\csname #1\endcsname}
\def\@eha{%
  Your command was ignored.^^J
  Type \space I <command> <return> \space to replace
  it with another command,^^J
  or \space <return> \space to continue without it.}
\def\@spaces{\space\space\space\space}
\def\typeout#1{\immediate\write\@unused{#1}}
\alloc@7\write\chardef\sixt@@n\@unused
\def\@empty{}
\def\@gobble#1{}
\def\@nnil{\@nil}
\def\@ifnextchar#1#2#3{%
\let\@tempe#1\def\@tempa{#2}\def\@tempb{#3}\futurelet\@tempc\@ifnch}
\def\@ifnch{%
  \ifx\@tempc\@sptoken
    \let\@tempd\@xifnch
  \else
    \ifx\@tempc\@tempe \let\@tempd\@tempa \else \let\@tempd\@tempb \fi
  \fi
  \@tempd}
\begingroup
\def\:{\global\let\@sptoken= } \:
\def\:{\@xifnch} \expandafter\gdef\: {\futurelet\@tempc\@ifnch}
\endgroup
\fi
\typeout{`PSTricks' v\fileversion\space\space <\filedate> (tvz)}
\def\@pstrickserr#1#2{%
  \begingroup
  \newlinechar`\^^J
  \edef\pst@tempc{#2}%
  \expandafter\errhelp\expandafter{\pst@tempc}%
  \typeout{%
    PSTricks error. \space See User's Guide for further information.^^J
    \@spaces\@spaces\@spaces\@spaces
    Type \space H <return> \space for immediate help.}%
  \errmessage{#1}%
  \endgroup}
\def\@ehpa{%
  Your command was ignored. Default value substituted.^^J
  Type \space <return> \space to procede.}
\def\@ehpb{%
  Your command was ignored. Will recover best I can.^^J
  Type \space <return> \space to procede.}
\def\@ehpc{%
  You better fix this before proceding.^^J
  See the PSTricks User's Guide or ask your system administrator for help.^^J
  Type \space X <return> \space to quit.}
\def\pst@misplaced#1{\@pstrickserr{Misplaced \string#1 command}\@ehpb}
\newdimen\pst@dima
\newdimen\pst@dimb
\newdimen\pst@dimc
\newdimen\pst@dimd
\newdimen\pst@dimg
\newdimen\pst@dimh
\newbox\pst@hbox
\newbox\pst@boxg
\newcount\pst@cnta
\newcount\pst@cntb
\newcount\pst@cntc
\newcount\pst@cntd
\newcount\pst@cntg
\newcount\pst@cnth
\newif\if@pst
\newtoks\pst@toks
\newif\if@star
\def\pst@ifstar#1{%
  \@ifnextchar*{\@startrue\def\next*{#1}\next}{\@starfalse#1}}
\def\pst@expandafter#1#2{%
  \def\next{#1}%
  \edef\@tempa{#2}%
  \ifx\@tempa\@empty
    \@pstrickserr{Unexpected empty argument!}\@ehpb
    \def\@tempa{\@empty}%
  \fi
  \expandafter\next\@tempa}
\def\pst@dimtonum#1#2{\edef#2{\pst@@dimtonum#1}}
\def\pst@@dimtonum#1{\expandafter\pst@@@dimtonum\the#1}
{\catcode`\p=12 \catcode`\t=12 \global\@namedef{pst@@@dimtonum}#1pt{#1}}
%
\def\pst@pyth#1#2#3{% from pst-3d
  \begingroup
    \pst@dima=#1\relax
    \ifnum\pst@dima<\z@\pst@dima=-\pst@dima\fi  % dima=abs(x)
    \pst@dimb=#2\relax
    \ifnum\pst@dimb<\z@\pst@dimb=-\pst@dimb\fi  % dimb=abs(y)
    \advance\pst@dimb\pst@dima         % dimb=s=abs(x)+abs(y)
    \ifnum\pst@dimb=\z@
      \global\pst@dimg=\z@             % dimg=z=sqrt(x^2+y^2)
    \else
      \multiply\pst@dima 8\relax              % dima= 8abs(x)
      \pst@@divide\pst@dima\pst@dimb     % dimg =8t=8abs(x)/s
      \advance\pst@dimg -4pt            % dimg = 4tau = (8t-4)
      \multiply\pst@dimg 2
      \pst@dimtonum\pst@dimg\pst@tempa
      \pst@dima=\pst@tempa\pst@dimg           % dima=(8tau)^2
      \advance\pst@dima 64pt         % dima=u=[64+(8tau)^2]/2
      \divide\pst@dima 2\relax                      % =(8f)^2
      \pst@dimd=7pt                % initial guess at sqrt(u)
      \pst@@pyth\pst@@pyth\pst@@pyth            % dimd=sqrt(u)
      \pst@dimtonum\pst@dimd\pst@tempa
      \pst@dimg=\pst@tempa\pst@dimb
      \global\divide\pst@dimg 8             % dimg=z=(8f)*s/8
    \fi
  \endgroup
  #3=\pst@dimg}
\def\pst@@pyth{%                      dimd = g <-- (g + u/g)/2
  \pst@@divide\pst@dima\pst@dimd
  \advance\pst@dimd\pst@dimg
  \divide\pst@dimd 2\relax}
%
% ----- the old pst@pyth begin -----
\iffalse
\def\pst@pyth#1#2#3{\ifdim#1>#2\pst@@pyth#1#2#3\else\pst@@pyth#2#1#3\fi}
\def\pst@@pyth#1#2#3{%
  \ifdim4#1>9#2%
    #3=#1\advance#3 .2122#2%
  \else
    #3=.8384#1\advance#3 .5758#2%
  \fi%
}
\fi
% ----- the old pst@pyth end -----
%
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \pst@dimtonum\pst@dimg{#3}%
}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax
  \pst@dimh=#2\relax
  \pst@cntg=\pst@dimh
  \pst@cnth=67108863
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide
  \divide\pst@dimg\pst@cntg%
}
\def\pst@@@divide{%
  \ifnum
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cnth
      \multiply\pst@dimg\sixt@@n
    \else
      \divide\pst@cntg\sixt@@n
    \fi%
}
\def\pst@configerr#1{%
  \@pstrickserr{\string#1 not defined in pstricks.con}\@ehpc}
%
\def\pstVerb#1{\pst@configerr\pstVerb}
\def\pstverb#1{\pst@configerr\pstverb}
\def\pstverbscale{\pst@configerr\pstverbscale}
\def\pstrotate{\pst@configerr\pstrotate}
\def\pstheader#1{\pst@configerr\pstheader}
\def\pstdriver{\pst@configerr\pstdriver}
\@ifundefined{pstcustomize}%
{\def\pstcustomize{\endinput\let\pstcustomize\relax}}{}
\input pstricks.con
\newif\ifPSTricks
\PSTrickstrue
\def\PSTricksOff{%
  \def\pstheader##1{}%
  \def\pstverb##1{}%
  \def\pstVerb##1{}%
  \PSTricksfalse%
}
\@ifundefined{pst@def}{\def\pst@def#1<#2>{\@namedef{tx@#1}{#2 }}}{}
\@ifundefined{pst@ATH}{\def\pst@ATH<#1>{}}{}
\pstheader{pstricks.pro}
\def\pst@dict{tx@Dict begin }
\def\pst@theheaders{pstricks.pro}
\def\pst@Verb#1{\pstVerb{\pst@dict #1 end}}
\def\tx@Atan{Atan }
\def\tx@Div{Div }
\def\tx@NET{NET }
\def\tx@Pyth{Pyth }
\def\tx@PtoC{PtoC }
\def\tx@PathLength@{PathLength@ }
\def\tx@PathLength{PathLength }
\pst@dimg=\pstunit\relax
\ifdim\pst@dimg=1bp
\def\pst@stp{.996264 dup scale}
\else
\edef\pst@stp{1 \pst@@dimtonum\pst@dimg\space div dup scale}
\fi
\def\tx@STP{STP }
\def\tx@STV{STV }
\def\pst@number#1{\pst@@dimtonum#1\space}
\def\pst@checknum#1#2{%
  \edef\next{#1}%
  \ifx\next\@empty
    \let\pst@num\z@
  \else
    \expandafter\pst@@checknum\next..\@nil
  \fi
  \ifnum\pst@num=\z@
    \@pstrickserr{Bad number: `#1'. 0 substituted.}\@ehpa
    \def#2{0 }%
  \else
    \edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
    \expandafter\@gobble\the\pst@cnth\space}%
  \fi}
\def\pst@@checknum{%
  \@ifnextchar-%
  {\let\pst@num\tw@\expandafter\pst@@@checknum\@gobble}%
  {\let\pst@num\@ne\pst@@@checknum}%
}
\def\pst@@@checknum#1.#2.#3\@nil{%
\afterassignment\pst@@@@checknum\pst@cntg=0#1\relax\@nil
\afterassignment\pst@@@@checknum\pst@cnth=1#2\relax\@nil}
\def\pst@@@@checknum#1\relax\@nil{%
\ifx\@nil#1\@nil\else\let\pst@num\z@\fi}
\def\pst@getnumii#1 #2 #3\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph}
\def\pst@getnumiii#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi}
\def\pst@getnumiv#1 #2 #3 #4 #5\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi
\pst@checknum{#4}\pst@tempj}
\def\pst@getdimnum#1 #2 #3\@nil{%
  \pssetlength\pst@dimg{#1}%
  \pst@checknum{#2}\pst@tempg%
}
% DG/SR modification begin - Jan. 7, 1998 - Patch 9
% Missing from pstricks.bug 0.93
%\def\pst@getscale#1#2{%
%\pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
%\@psttrue
%\ifdim\pst@tempg\p@=\z@
%\@pstrickserr{Bad scaling argument `#1'}\@ehpa
%\def\pst@tempg{1 }%
%\@pstfalse
%\fi
%\ifdim\pst@temph\p@=\z@
%\if@pst\@pstrickserr{Bad scaling argument `#1'}\@ehpa\fi
%\def\pst@temph{1 }%
%\fi
%\edef#2{\pst@tempg\space \pst@temph\space scale }%
%\ifdim\pst@tempg\p@=\p@ \ifdim\pst@temph\p@=\p@
%\def#2{}%
%\fi\fi}
\def\pst@getscale#1#2{%
  \edef\pst@tempg{#1}%
  \ifx\pst@tempg\@none
    \def#2{}%
  \else
    \pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
    \ifdim\pst@tempg\p@=\z@
      \@pstrickserr{Bad scaling argument `#1'}\@ehpa
      \def#2{}%
    \else
      \ifdim\pst@temph\p@=\z@
        \@pstrickserr{Bad scaling argument `#1'}\@ehpa
        \def#2{}%
      \else
        \edef#2{\pst@tempg\space \pst@temph\space scale }%
      \fi
    \fi
  \fi%
}
% DG/SR modification end
\def\pst@getint#1#2{%
  \pst@cntg=#1\relax
  \edef#2{\the\pst@cntg\space}%
}
\begingroup
\catcode`\{=12
\catcode`\}=12
\catcode`\[=1
\catcode`\]=2
\gdef\pslbrace[{ ]
\gdef\psrbrace[} ]
\endgroup
\def\@newcolor#1#2{%
\expandafter\edef\csname #1\endcsname{\noexpand\pst@color{#2}}%
%\expandafter\edef\csname color@#1\endcsname{#2}%
\expandafter\edef\csname\string\color@#1\endcsname{#2}%    hv 1.14 2005-12-17
\ignorespaces}
\def\pst@color#1{%
\def\pst@currentcolor{#1}\pstVerb{#1}\aftergroup\pst@endcolor}
\def\pst@endcolor{\pstVerb{\pst@currentcolor}}
\def\pst@currentcolor{0 setgray}
\def\altcolormode{%
\def\pst@color##1{%
\pstVerb{gsave ##1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@grestore}}}
\def\pst@grestore{%
  currentpoint
  matrix currentmatrix
  currentfont
  grestore
  setfont
  setmatrix
  moveto
}
%\def\pst@usecolor#1{\csname color@#1\endcsname\space}%    hv 1.14  2005--12-17
\def\pst@usecolor#1{\csname\string\color@#1\endcsname\space}
%
\def\newgray#1#2{%
  \pst@checknum{#2}\pst@tempg
  \@newcolor{#1}{\pst@tempg setgray}}
\def\newrgbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi setrgbcolor}}
\def\newhsbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi sethsbcolor}}
\def\newcmykcolor#1#2{%
  \pst@expandafter\pst@getnumiv{#2} {} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi \pst@tempj setcmykcolor}}
\newgray{black}{0}
\newgray{darkgray}{.25}
\newgray{gray}{.5}
\newgray{lightgray}{.75}
\newgray{white}{1}
\newrgbcolor{red}{1 0 0}
\newrgbcolor{green}{0 1 0}
\newrgbcolor{blue}{0 0 1}
\newrgbcolor{yellow}{1 1 0}
\newrgbcolor{cyan}{0 1 1}
\newrgbcolor{magenta}{1 0 1}
\def\psset#1{\@psset#1,\@nil\ignorespaces}
\def\@psset#1,{%
  \@@psset#1==\@nil%
  \@ifnextchar\@nil{\@gobble}{\@psset}%
}
\def\@@psset#1=#2=#3\@nil{%
  \@ifundefined{psset@#1}%
    {\@pstrickserr{Graphics parameter `#1' not defined.}\@ehpa}%
    {\@nameuse{psset@#1}{#2}}%
}%
\def\psset@style#1{%
  \@ifundefined{pscs@#1}%
    {\@pstrickserr{Custom style `#1' undefined}\@ehpa}%
    {\@nameuse{pscs@#1}}%
}
%\def\newpsstyle#1#2{\@namedef{pscs@#1}{\psset{#2}}}
%------------ hv 1.10 beg -------------------
\def\newpsstyle#1#2{\@namedef{pscs@#1}{%
  \def\pst@tempa{#2}%
  \ifx\pst@tempa\@empty\else\psset{#2}\fi}}
%------------ hv 1.10 end -------------------
\def\@none{none}
\def\pst@getcolor#1#2{%
%  \@ifundefined{color@#1}%	hv 1.14  2005-12-17
  \@ifundefined{\string\color@#1}%
    {\@pstrickserr{Color `#1' not defined}\@eha}%
    {\edef#2{#1}}%
}
\newdimen\psunit \psunit 1cm
\newdimen\psxunit \psxunit 1cm
\newdimen\psyunit \psyunit 1cm
\let\psrunit\psunit
\def\pstunit@off{\let\@psunit\ignorespaces\ignorespaces}
\def\pssetlength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\psaddtolength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  \advance#1 #2\@psunit%
}
\def\pssetxlength#1#2{%
  \let\@psunit\psxunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\pssetylength#1#2{%
  \let\@psunit\psyunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\psset@unit#1{%
  \pssetlength\psunit{#1}%
  \psxunit=\psunit
  \psyunit=\psunit%
}
\def\psset@runit#1{\pssetlength\psrunit{#1}}
\def\psset@xunit#1{\pssetxlength\psxunit{#1}}
\def\psset@yunit#1{\pssetylength\psyunit{#1}}
% v 1.05   begin
\def\psset@PstDebug#1{\pst@getint{#1}{\Pst@Debug}}% hv 2004-06-22
\psset{PstDebug=0}
% end
\def\pst@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\pst@number\pst@dimg}%
}
\def\pst@@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\number\pst@dimg sp}%
}
\def\pst@getcoor#1#2{\pst@@getcoor{#1}\let#2\pst@coor}
\def\pst@coor{0 0 }
\def\pst@getcoors#1#2{%
  \def\pst@aftercoors{\addto@pscode{#1 \pst@coors }#2}%
  \def\pst@coors{}%
  \pst@@getcoors%
}
\def\pst@@getcoors(#1){%
  \pst@@getcoor{#1}%
  \edef\pst@coors{\pst@coor\pst@coors}%
  \@ifnextchar({\pst@@getcoors}{\pst@aftercoors}%
}
\def\pst@getangle#1#2{\pst@@getangle{#1}\let#2\pst@angle}
\def\pst@angle{0 }
\def\cartesian@coor#1,#2,#3\@nil{%
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
}
\def\NormalCoor{%
  \def\pst@@getcoor##1{\pst@expandafter\cartesian@coor{##1},\relax,\@nil}%
  \def\pst@@getangle##1{%
    \pst@checknum{##1}\pst@angle
    \edef\pst@angle{\pst@angle \pst@angleunit}%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@cartesian}%
}
\NormalCoor
\def\degrees{\@ifnextchar[{\@degrees}{\def\pst@angleunit{}}}
\def\@degrees[#1]{%
\pst@checknum{#1}\pst@tempg
\edef\pst@angleunit{360 \pst@tempg div mul }%
\ignorespaces}
\def\radians{\def\pst@angleunit{57.2956 mul }}
\def\pst@angleunit{}
\def\SpecialCoor{%
  \def\pst@@getcoor##1{%
    \begingroup
      \pst@activecoor
      \xdef\pst@tempg{##1}%
    \endgroup
    \expandafter\special@coor\pst@tempg||\@nil%
  }%
  \def\pst@@getangle##1{%
    \begingroup
      \pst@activecoor
      \xdef\pst@tempg{##1}%
    \endgroup
    \expandafter\special@angle\pst@tempg\@empty)\@nil%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@special}%
}
\begingroup
\catcode`\|=13
\catcode`\;=13
\catcode`\!=13
\gdef\pst@activecoor{%
  \def|{\string|}%
  \def;{\string;}%
  \def!{\string!}%
}
\endgroup
\def\special@coor#1|#2|#3\@nil{%
  \ifx#3|\relax
    \mixed@coor{#1}{#2}%
  \else
    \special@@coor#1;;\@nil
  \fi%
}
\def\special@@coor#1{%
  \ifcat#1a\relax
    \def\next{\node@coor#1}%
  \else
    \ifx#1[\relax
      \def\next{\Node@coor[}%
    \else
      \ifx#1!\relax
        \def\next{\raw@coor}%
      \else
        \def\next{\special@@@coor#1}%
      \fi
    \fi
  \fi
  \next%
}
\def\special@@@coor#1;#2;#3\@nil{%
  \ifx#3;\relax
    \polar@coor{#1}{#2}%
  \else
    \cartesian@coor#1,\relax,\@nil
  \fi%
}
\def\mixed@coor#1#2{%
  \begingroup
% DG/SR modification begin - Oct. 27, 1997 - Patch 6
%\specialcoor@ii#1;;\@nil
%\let\pst@tempa\pst@coor
%\specialcoor@ii#2;;\@nil
    \special@@coor#1;;\@nil
    \let\pst@tempa\pst@coor
    \special@@coor#2;;\@nil
% DG/SR modification end
    \xdef\pst@tempg{\pst@tempa pop \pst@coor exch pop }%
  \endgroup
  \let\pst@coor\pst@tempg%
}
\def\polar@coor#1#2{%
  \pssetlength\pst@dimg{#1}%
  \pst@@getangle{#2}%
  \edef\pst@coor{\pst@number\pst@dimg \pst@angle \tx@PtoC}%
}
\def\raw@coor#1;#2\@nil{%
  \edef\pst@coor{%
    #1 \pst@number\psyunit mul exch \pst@number\psxunit mul exch }%
}
\def\node@coor#1\@nil{%
  \@pstrickserr{You must load `pst-node.tex' to use node coordinates.}\@ehps
  \def\pst@coor{0 0 }%
}
\def\Node@coor{\node@coor}
\def\special@angle#1#2)#3\@nil{%
\ifx!#1\relax
\edef\pst@angle{#2 \pst@angleunit}%
\else
\ifx(#1\relax
\pst@@getcoor{#2}%
\edef\pst@angle{\pst@coor exch \tx@Atan}%
\else
\pst@checknum{#1#2}\pst@angle
\edef\pst@angle{\pst@angle \pst@angleunit}%
\fi
\fi}
\def\Cartesian{%
  \def\cartesian@coor##1,##2,##3\@nil{%
    \pssetxlength\pst@dimg{##1}%
    \pssetylength\pst@dimh{##2}%
    \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
  }%
  \@ifnextchar({\Cartesian@}{}%
}
\def\Cartesian@(#1,#2){%
  \pssetxlength\psxunit{#1}%
  \pssetylength\psyunit{#2}%
  \ignorespaces%
}
\def\Polar{%
  \def\psput@cartesian{\psput@special}%
  \def\cartesian@coor##1,##2,##3\@nil{\polar@coor{##1}{##2}}%
}%
\def\psset@origin#1{%
  \pst@@getcoor{#1}%
% ----------- 1.10 beg hv -------------------
%  \edef\psk@origin{\pst@coor \tx@NET }}
  \edef\psk@origin{\pst@coor T }}
% ----------- 1.10 end hv -------------------
\def\psk@origin{}
%
\newif\ifswapaxes
\def\psset@swapaxes#1{%
  \@nameuse{@pst#1}%
  \if@pst\def\psk@swapaxes{-90 rotate -1 1 scale }%
  \else\def\psk@swapaxes{}%
  \fi%
}
\psset@swapaxes{false}
\newif\ifshowpoints
\def\psset@showpoints#1{\@nameuse{showpoints#1}}
\psset@showpoints{false}
\let\pst@setrepeatarrowsflag\relax
\def\psset@border#1{%
\pst@getlength{#1}\psk@border
\pst@setrepeatarrowsflag}
\psset@border{0pt}
\def\psset@bordercolor#1{\pst@getcolor{#1}\psbordercolor}
\psset@bordercolor{white}
\newif\ifpsdoubleline
\def\psset@doubleline#1{%
  \@nameuse{psdoubleline#1}%
  \pst@setrepeatarrowsflag}
\psset@doubleline{false}
\def\psset@doublesep#1{\def\psdoublesep{#1}}
\psset@doublesep{1.25\pslinewidth}
\def\psset@doublecolor#1{\pst@getcolor{#1}\psdoublecolor}
\psset@doublecolor{white}
\newif\ifpsshadow
\def\psset@shadow#1{%
  \@nameuse{psshadow#1}%
  \pst@setrepeatarrowsflag}
\psset@shadow{false}
\def\psset@shadowsize#1{\pst@getlength{#1}\psk@shadowsize}
\psset@shadowsize{3pt}
\def\psset@shadowangle#1{\pst@getangle{#1}\psk@shadowangle}
\psset@shadowangle{-45}
\def\psset@shadowcolor#1{\pst@getcolor{#1}\psshadowcolor}
\psset@shadowcolor{darkgray}
\def\pst@repeatarrowsflag{\z@}
\def\pst@setrepeatarrowsflag{%
  \edef\pst@repeatarrowsflag{%
    \ifdim\psk@border\p@>\z@ 1\else\ifpsdoubleline 1\else
      \ifpsshadow 1\else \z@\fi\fi\fi}}
\def\psls@none{}
\newdimen\pslinewidth
\def\psset@linewidth#1{\pssetlength\pslinewidth{#1}}
\psset@linewidth{.8pt}
\def\psset@linecolor#1{\pst@getcolor{#1}\pslinecolor}
\psset@linecolor{black}
\def\psls@solid{0 setlinecap stroke }
\def\pst@missing{%
  \z@
  \@pstrickserr{Missing number or dimension. 0 substituted}\@ehpa}
%
%%------------------- begin patch 15 HV 2004-05-15 -------------
%\def\psset@dash#1{%
%  \pst@expandafter\psset@@dash{#1} {\pst@missing} {\pst@missing} {}\@nil
%  \edef\psk@dash{\pst@number\pst@dimg \pst@number\pst@dimh}%
%}
%\def\psset@@dash#1 #2 #3\@nil{%
%\pssetlength\pst@dimg{#1}%
%\pssetlength\pst@dimh{#2}}
%\psset@dash{5pt 3pt}
\def\pst@empty{\z@}
\def\psset@dash#1{% black white [ black white ] 
  \pst@expandafter\psset@@dash{#1} {\pst@empty} {\pst@empty} %
                  {\pst@missing} {\pst@missing} {}\@nil
  \edef\psk@dash{\pst@number\pst@dimg \pst@number\pst@dimh 
                 \pst@number\pst@dimc \pst@number\pst@dimd}%
}
\def\psset@@dash#1 #2 #3 #4 #5\@nil{% 
  \pssetlength\pst@dimg{#1}%
  \pssetlength\pst@dimh{#2}%
  \pssetlength\pst@dimc{#3}%
  \pssetlength\pst@dimd{#4}%
}
\psset@dash{5pt 3pt 0pt 0pt}% black white black white 
%%------------------- end patch 15 HV 2004-05-15 -------------
\newif\ifpsdashadjust
\def\psset@dashadjust#1{\@nameuse{psdashadjust#1}}
\psset@dashadjust{true}
\def\tx@DashLine{DashLine }
\def\psls@dashed{%
%%--------------------------------- hv 2006-04-29 beg ---------------------
  \psk@linecap\space setlinecap
%%--------------------------------- hv 2006-04-29 end ---------------------
  \ifpsdashadjust
%    \psk@dash \pst@linetype\space \tx@DashLine
    \psk@dash \@ifundefined{pst@linetype}{2}{\pst@linetype}\space \tx@DashLine
  \else
    [ \psk@dash ] 0 setdash stroke
  \fi}
\def\psset@dotsep#1{\pst@getlength{#1}\psk@dotsep}
\psset@dotsep{3pt}
\def\tx@DotLine{DotLine }
\def\psls@dotted{%
  \ifpsdashadjust
    \psk@dotsep \pst@linetype\space \tx@DotLine
  \else
    [ 0 \psk@dotsep CLW add ] 0 setdash 1 setlinecap stroke
  \fi%
}
\def\psset@linestyle#1{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\edef\pslinestyle{#1}}%
}
\psset@linestyle{solid}
%%--------------------------------- hv 2006-04-29 beg ---------------------
\def\psset@linecap#1{%
  \def\psk@linecap{0}%
  \ifnum#1>-1
    \ifnum#1<3
      \pst@getint{#1}\psk@linecap%
  \fi\fi%
}
\psset{linecap=0}
%%--------------------------------- hv 2006-04-29 end ---------------------

\def\psfs@none{}
\def\psset@fillcolor#1{\pst@getcolor{#1}\psfillcolor}
\psset@fillcolor{white}
\def\psfs@solid{\pst@fill{\pst@usecolor\psfillcolor fill}}
%-------------- hv begin patch 15 (2004-05-10)---------------%%
\def\psfs@eofill{\pst@fill{\pst@usecolor\psfillcolor eofill}}
%-------------- hv end patch 15  (2004-05-10)---------------%%
\def\psset@hatchwidth#1{\pst@getlength{#1}\psk@hatchwidth}
\psset@hatchwidth{.8pt}
\def\psset@hatchsep#1{\pst@getlength{#1}\psk@hatchsep}
\psset@hatchsep{4pt}
\def\psset@hatchcolor#1{\pst@getcolor{#1}\pshatchcolor}
\psset@hatchcolor{black}
\def\psset@hatchangle#1{\pst@getangle{#1}\psk@hatchangle}
\psset@hatchangle{45}
% ------------ hv 1.11 ------------
\def\psset@hatchsepinc#1{\pst@getlength{#1}\psk@hatchsepinc}
\def\psset@hatchwidthinc#1{\pst@getlength{#1}\psk@hatchwidthinc}
\psset@hatchwidthinc{0pt}
\psset@hatchsepinc{0pt}
%
\def\pst@linefill{%
  \psk@hatchangle rotate
  \psk@hatchwidth SLW
  \pst@usecolor\pshatchcolor
  \psk@hatchsep 
  \psk@hatchsepinc
  \psk@hatchwidthinc
  \tx@LineFill }
% ------------ hv 1.11 ------------
%
\def\psfs@vlines{\pst@fill\pst@linefill}
\@namedef{psfs@vlines*}{\psfs@solid \psfs@vlines}
\def\psfs@hlines{\pst@fill{90 rotate \pst@linefill}}
\@namedef{psfs@hlines*}{\psfs@solid \psfs@hlines}
\def\psfs@crosshatch{\psfs@vlines \psfs@hlines}
\@namedef{psfs@crosshatch*}{\psfs@solid \psfs@vlines \psfs@hlines}
\def\tx@LineFill{LineFill }
\def\psset@fillstyle#1{%
  \edef\pst@tempg{#1}\def\pst@temph{none}%
  \ifx\pst@tempg\pst@temph
     \let\psk@fillstyle\relax
  \else
    \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{\expandafter\noexpand\csname psfs@#1\endcsname}}%
  \fi%
}
\def\psset@addfillstyle#1{%
  \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{%
      \expandafter\noexpand\psk@fillstyle
      \expandafter\noexpand\csname psfs@#1\endcsname}%
    }%
}
\psset@fillstyle{none}
\def\psset@arrows#1{%
  \begingroup
    \pst@activearrows
    \xdef\pst@tempg{#1}%
  \endgroup
  \expandafter\psset@@arrows\pst@tempg\@empty-\@empty\@nil
  \if@pst\else
    \@pstrickserr{Bad arrows specification: #1}\@ehpa
  \fi%
}
\def\psset@@arrows#1-#2\@empty#3\@nil{%
  \@psttrue
  \def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
  \expandafter\next\pst@arrowtable,#1-#1,\@nil
  \@ifundefined{psas@\pst@tempg}%
    {\@pstfalse\def\psk@arrowA{}}%
    {\let\psk@arrowA\pst@tempg}%
  \@ifundefined{psas@#2}%
    {\@pstfalse\def\psk@arrowB{}}%
    {\def\psk@arrowB{#2}}%
}
\def\psk@arrowA{}
\def\psk@arrowB{}
%\def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-]}
\def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-],)-(,]-[,|>-<|} % hv --1.12
\begingroup
  \catcode`\<=13
  \catcode`\>=13
  \catcode`\|=13
  \gdef\pst@activearrows{\def<{\string<}\def>{\string>}\def|{\string|}}
\endgroup
\def\tx@BeginArrow{BeginArrow }
\def\tx@EndArrow{EndArrow }
% Redefininition of \psset@arrowscale to store value of X scale factor  hv --1.12
%\def\psset@arrowscale#1{\pst@getscale{#1}\psk@arrowscale}
\def\psset@arrowscale#1{%                                   hv --1.12
  \pst@@arrowscale@i#1 \@nil%                               hv -- 1.12 
  \pst@getscale{\pst@arrowscale}\psk@arrowscale}%           hv --1.12
\def\pst@@arrowscale@i#1 #2\@nil{\edef\pst@arrowscale{#1}}% hv --1.12
\psset@arrowscale{1}
%
\def\psset@arrowsize#1{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@arrowsize{\pst@number\pst@dimg \pst@tempg}%
}
\psset@arrowsize{1.5pt 2}
\def\psset@arrowlength#1{\pst@checknum{#1}\psk@arrowlength}
\psset@arrowlength{1.4}
\def\psset@arrowinset#1{\pst@checknum{#1}\psk@arrowinset}%
\psset@arrowinset{.4}
\def\tx@Arrow{Arrow }
% new definitions of the missing arrows ---- hv 1.1.2
\@namedef{psas@<|}{%
    \psk@tbarsize\space \tx@Tbar
    0 CLW 2 div T
    newpath
    true \psk@arrowinset\space \psk@arrowlength\space \psk@arrowsize\space \tx@Arrow%
}
% ]-[ arrow
\def\tx@BracketOut{BracketOut }
\@namedef{psas@[}{%
  /BracketOut {%
  CLW mul add dup CLW sub 2 div
%/x ED mul CLW add
  /x ED mul neg
  /y ED
  /z CLW 2 div def
  x neg y moveto
  x neg CLW 2 div L x CLW 2 div L x y L stroke 0 CLW moveto } def
  \psk@bracketlength\space \psk@tbarsize\space \tx@BracketOut
}
% )-( arrow
\def\tx@RoundBracketOut{RoundBracketOut }
\@namedef{psas@(}{%
  /RoundBracketOut {%
    CLW mul add dup 2 div
%/x ED mul
    /x ED mul neg
    /y ED
    /mtrx CM def
    0 CLW
    2 div T x y mul 0 ne { x y scale } if
    1 1 moveto
    .85 .5 .35 0 0 0 curveto
    -.35 0 -.85 .5 -1 1 curveto
    mtrx setmatrix stroke 0 CLW moveto } def
  \psk@rbracketlength\space \psk@tbarsize\space \tx@RoundBracketOut
}
% end of new definitions of the missing arrows ---- hv 1.12
\@namedef{psas@>}{%
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@>>}{%
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  0 h T
  gsave
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP
  grestore
  CP newpath moveto
  2 copy
  L
  stroke
  moveto
}
\@namedef{psas@<}{true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@<<}{%
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP newpath moveto 0 a neg L stroke 0 h neg T
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\def\psset@tbarsize#1{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@tbarsize{\pst@number\pst@dimg \pst@tempg}%
}
\psset@tbarsize{2pt 5}
\def\tx@Tbar{Tbar }
\@namedef{psas@|}{\psk@tbarsize \tx@Tbar}
\@namedef{psas@|*}{0 CLW -2 div T \psk@tbarsize \tx@Tbar}
\@namedef{psas@>|}{%
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@>|*}{%
  0 CLW -2 div T
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\edef\pst@arrowtable{\pst@arrowtable,|<*->|*,|<->|}
\def\psset@bracketlength#1{\pst@checknum{#1}\psk@bracketlength}
\psset@bracketlength{.15}
\def\tx@Bracket{Bracket }
\@namedef{psas@]}{\psk@bracketlength \psk@tbarsize \tx@Bracket}
\def\psset@rbracketlength#1{\pst@checknum{#1}\psk@rbracketlength}
\psset@rbracketlength{.15}
\def\tx@RoundBracket{RoundBracket }
\@namedef{psas@)}{\psk@rbracketlength \psk@tbarsize \tx@RoundBracket}
\def\psas@c{1 \psas@@c}
\def\psas@cc{0 CLW 2 div T 1 \psas@@c}
\def\psas@C{2 \psas@@c}
\def\psas@@c{%
  setlinecap
  0 0 moveto
%%-------------------- v.1.04 begin HV 2004-05-18 ----------------
%  0 CLW 2 div L
  0 0.1 L % changed value from 0.5 to 0.1
%%-------------------- v. 1.04 end HV 2004-05-18 ----------------
  stroke
  0 0 moveto
}
\def\psas@{}
\psset@arrows{-}
\def\tx@SD{SD }
\def\tx@EndDot{EndDot }
\def\psas@oo{{\pst@usecolor\psfillcolor true} true \psk@dotsize \tx@EndDot}
\def\psas@o{{\pst@usecolor\psfillcolor true} false \psk@dotsize \tx@EndDot}
\@namedef{psas@**}{{false} true \psk@dotsize \tx@EndDot}
\@namedef{psas@*}{{false} false \psk@dotsize \tx@EndDot}
\def\pst@par{}
\def\addto@par#1{%
\ifx\pst@par\@empty
\def\pst@par{#1}%
\else
\expandafter\def\expandafter\pst@par\expandafter{\pst@par,#1}%
\fi}
\def\addbefore@par#1{%
\ifx\pst@par\@empty
\def\pst@par{#1}%
\else
\toks@{#1}%
\pst@toks\expandafter{\pst@par}%
\edef\pst@par{\the\toks@,\the\pst@toks}%
\fi}
\def\use@par{%
  \ifx\pst@par\@empty\else
    \expandafter\@psset\pst@par,\@nil
    \def\pst@par{}%
  \fi%
}
\def\pst@object#1{%
  \pst@ifstar{%
    \@ifnextchar[{\pst@@object{#1}}{\def\pst@par{}\@nameuse{#1@i}}}%
}
\def\pst@@object#1[#2]{%
  \def\pst@par{#2}%
  \@ifnextchar+{\@nameuse{#1@i}}{\@nameuse{#1@i}}}
\def\newpsobject#1#2#3{%
\@ifundefined{#2@i}%
{\@pstrickserr{Graphics object `#2' not defined}\@eha}{%
\@namedef{#1}{\pst@object{#1}}%
\@namedef{#1@i}{\addbefore@par{#3}\@nameuse{#2@i}}}%
\ignorespaces}
\def\pst@getarrows#1{\@ifnextchar({#1}{\pst@@getarrows{#1}}}
% ------------------------- hv 1.10 beg ------------------------
%\def\pst@@getarrows#1#2{\addto@par{arrows=#2}#1}
\def\pst@@getarrows#1#2{%
  \def\pst@tempa{#2}% prevent empty arrow arguments, to allow \psline{}(...)(...)
  \ifx\pst@tempa\@empty\addto@par{arrows=-}\else\addto@par{arrows=#2}\fi#1}
% ------------------------- hv 1.10 end ------------------------
%
\def\begin@ClosedObj{%
  \leavevmode
  \pst@killglue
  \begingroup
    \use@par
    \solid@star
    \ifpsdoubleline \pst@setdoublesep \fi
    \init@pscode%
}
\def\end@ClosedObj{%
  \ifpsshadow \pst@closedshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifshowpoints
% DG modification begin - Mar. 4, 1995
%\addto@pscode{Points aload length 2 div cvi /N ED \psdots@iii}%
  \pst@OpenShowPoints
% DG modification end
  \fi
  \use@pscode
  \endgroup
  \ignorespaces%
}
\def\begin@OpenObj{%
  \begin@ClosedObj
  \let\pst@linetype\pst@arrowtype
  \pst@addarrowdef%
}
\def\begin@AltOpenObj{%
  \begin@ClosedObj
  \def\pst@repeatarrowsflag{\z@}%
  \def\pst@linetype{0}}
\def\end@OpenObj{%
  \ifpsshadow \pst@openshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifnum\pst@repeatarrowsflag>\z@ \pst@repeatarrows \fi
  \ifshowpoints \pst@OpenShowPoints \fi
  \use@pscode
  \endgroup
  \ignorespaces}
\def\begin@SpecialObj{%
\leavevmode
\pst@killglue
\begingroup
\use@par
\init@pscode}
\def\end@SpecialObj{%
\use@pscode
\endgroup
\ignorespaces}
\def\pst@code{}%
\def\init@pscode{%
  \addto@pscode{%
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor}%
}
\def\addto@pscode#1{\xdef\pst@code{\pst@code#1\space}}
\def\use@pscode{%
  \pstverb{%
    \pst@dict
    \tx@STP
    \pst@newpath
    \psk@origin
    \psk@swapaxes
    \pst@code
    end
  }%
  \gdef\pst@code{}%
}
\def\pst@newpath{newpath }
\def\pst@@killglue{\unskip\ifdim\lastskip>\z@\expandafter\pst@@killglue\fi}
\def\KillGlue{\let\pst@killglue\pst@@killglue}
\def\DontKillGlue{\let\pst@killglue\relax}
\DontKillGlue
\def\solid@star{%
  \if@star
    \pslinewidth=\z@
    \psdoublelinefalse
    \def\pslinestyle{none}%
    \def\psk@fillstyle{\psfs@solid}%
    \let\psfillcolor\pslinecolor
  \fi}
\def\pst@setdoublesep{%
\pst@getlength\psdoublesep\psdoublesep
\pslinewidth=2\pslinewidth
\advance\pslinewidth\psdoublesep\p@
\let\pst@setdoublesep\relax}
\def\tx@Shadow{Shadow }
\def\pst@closedshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    gsave fill grestore
    stroke
    grestore
    gsave
    \pst@usecolor\psfillcolor
    gsave fill grestore
    stroke
    grestore}}
\def\pst@openshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    \ifx\psk@fillstyle\relax\else
      gsave fill grestore
    \fi
    stroke}%
  \pst@repeatarrows%
  \addto@pscode{grestore}%
  \ifx\psk@fillstyle\relax\else
    \addto@pscode{%
      gsave
      \pst@usecolor\psfillcolor
      gsave fill grestore
      stroke
      grestore}%
  \fi}
\def\pst@addborder{%
  \addto@pscode{%
    gsave
    \psk@border 2 mul
    CLW add SLW
    \pst@usecolor\psbordercolor
    stroke
    grestore}}
\def\pst@stroke{%
  \ifx\pslinestyle\@none\else
    \addto@pscode{%
      gsave
      \pst@number\pslinewidth SLW
      \pst@usecolor\pslinecolor
      \@nameuse{psls@\pslinestyle}
      grestore}%
  \fi}
\def\pst@fill#1{\addto@pscode{gsave #1 grestore}}%
\def\pst@doublestroke{%
    \addto@pscode{%
      gsave
      \psdoublesep SLW
      \pst@usecolor\psdoublecolor
      stroke
      grestore
    }}
\def\pst@arrowtype{%
\ifx\psk@arrowB\@empty 0 \else -2 \fi
\ifx\psk@arrowA\@empty 0 \else -1 \fi
add}
\def\pst@addarrowdef{%
\addto@pscode{%
/ArrowA {
\ifx\psk@arrowA\@empty
  \pst@oplineto
\else
  \pst@arrowdef{A}
moveto
\fi
} def
/ArrowB {
\ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi
} def}}
\def\pst@arrowdef#1{%
\ifnum\pst@repeatarrowsflag>\z@
/Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
\fi
\tx@BeginArrow
\psk@arrowscale
\@nameuse{psas@\@nameuse{psk@arrow#1}}
\tx@EndArrow}
\def\pst@repeatarrows{%
\addto@pscode{%
gsave
\ifx\psk@arrowA\@empty\else
ArrowAc ArrowA pop pop
\fi
\ifx\psk@arrowB\@empty\else
ArrowBc ArrowB pop pop pop pop
\fi
grestore}}
\def\pst@OpenShowPoints{%
  \addto@pscode{%
    gsave
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    newpath
    Points aload length 2 div 2 sub cvi /N ED
    N 0 ge
      { \ifx\psk@arrowA\@empty Dot \else pop pop \fi 
        N { Dot } repeat 
	\ifx\psk@arrowB\@empty Dot \else pop pop \fi }
      { N 2 mul { pop } repeat } ifelse
    grestore
}}
\def\pscustom{\pst@object{pscustom}}
\long\def\pscustom@i#1{%
  \begin@SpecialObj
  \solid@star
  \let\pst@ifcustom\iftrue
  \let\begin@ClosedObj\begin@CustomObj
  \let\end@ClosedObj\endgroup
  \def\begin@OpenObj{\begin@CustomObj\pst@addarrowdef}%
  \let\end@OpenObj\endgroup
  \let\begin@AltOpenObj\begin@CustomObj
  \def\begin@SpecialObj{%
    \begingroup
    \pst@misplaced{special graphics object}%
    \def\addto@pscode####1{}
    \let\end@SpecialObj\endgroup}%
    \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
    \def\psclip##1{\pst@misplaced\psclip}%
    \def\pst@repeatarrowsflag{\z@}%
    \let\pst@setrepeatarrowsflag\relax
    \showpointsfalse
    \let\showpointstrue\relax
    \def\pst@linetype{\pslinetype}%
    \let\psset@liftpen\psset@@liftpen
    \psset@liftpen{\z@}%
    \def\pst@cp{/currentpoint load stopped pop }%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
    \def\pst@optcp##1##2{%
    \ifnum##1=\z@\def##2{/currentpoint load stopped { 0 0 } if }\fi}%
    \let\caddto@pscode\addto@pscode
    \def\cuse@par##1{{\use@par##1}}%
    \the\pst@customdefs
    \setbox\pst@hbox=\hbox{#1}%
    \psk@fillstyle
    \pst@stroke
  \end@SpecialObj}
\def\begin@CustomObj{%
  \begingroup
  \use@par
  \addto@pscode{%
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor
  }%
}
\def\pst@oplineto{moveto }
\def\pst@cp{}
\def\pst@optcp#1#2{}
\def\psset@liftpen#1{}
\def\psset@@liftpen#1{%
  \ifcase#1\relax
    \def\psk@liftpen{\z@}%
    \def\pst@cp{/currentpoint load stopped pop }%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or
    \def\psk@liftpen{1}%
    \def\pst@cp{}%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or
    \def\psk@liftpen{2}%
    \def\pst@cp{}%
    \def\pst@oplineto{moveto }%
  \fi%
}
\psset@liftpen{0}
\def\psk@liftpen{-1}
%
\def\psset@linetype#1{%
  \pst@getint{#1}\pslinetype
%----------------- hv begin 2006-04-20 ------------- patch 1.14b
  \ifnum\pst@cntg<-3
%  \ifnum\pst@dimg<-3
%----------------- hv end 2004-05-07 ------------- patch 1.14b
    \@pstrickserr{linetype must be greater than -3}\@ehpa
%----------------- hv begin 2004-05-07 ------------- patch 15
%	\def\pslinetype{0}%
    \def\pslinetype{2}%
  \fi%
}
%\psset@linetype{0}
\psset@linetype{2}% otherwise there is a problem when using e.g.
%                     \psaxes[axesstyle=frame,linestyle=dashed]{->}(3,-2)
%----------------- hv end 2004-05-07 ------------- patch 15
%
\def\caddto@pscode#1{%
    \@pstrickserr{Command can only be used in \string\pscustom}\@ehpa%
}
\let\cuse@par\caddto@pscode
%
\def\tx@MSave{%
     /msavematrx
         [ tx@Dict /msavematrx known % does msavematrix exists?
             { msavematrx aload pop } if
             CM % matrix currentmatrix
         ]
     def
%----------------- hv begin 2004-05-07 ------------- patch 15
    msavematrx
%----------------- hv end 2004-05-07 ------------- patch 15
}
\def\tx@MRestore{% a typo in pstricks with msavematrx
     tx@Dict /msavematrx known { length 0 gt } { false } ifelse
         { msavematrx aload pop setmatrix } if
}
%
\newtoks\pst@customdefs
\pst@customdefs{%
  \def\newpath{\addto@pscode{newpath}}%
  \def\moveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
  \def\closepath{\addto@pscode{closepath}}%
  \def\gsave{\begingroup\addto@pscode{gsave}}%
  \def\grestore{\endgroup\addto@pscode{grestore}}%
% DG/SR modification begin - May 12, 1997 - Patch 2
%  \def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
  \def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor translate}}%
% DG/SR modification end
  \def\rotate#1{\pst@@getangle{#1}\addto@pscode{\pst@angle rotate}}%
  \def\scale#1{\pst@getscale{#1}\pst@tempg\addto@pscode{\pst@tempg}}%
  \def\msave{\addto@pscode{\tx@MSave}}%
  \def\mrestore{\addto@pscode{\tx@MRestore}}%
  \def\swapaxes{\addto@pscode{-90 rotate -1 1 scale}}%
  \def\stroke{\pst@object{stroke}}%
  \def\fill{\pst@object{fill}}%
  \def\openshadow{\pst@object{openshadow}}%
  \def\closedshadow{\pst@object{closedshadow}}%
% DG/SR modification begin - Jan. 7, 1998 - Patch 8
% \def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor tx@Shadow}}%
  \def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor \tx@Shadow}}%
% DG/SR modification end
  \def\lineto{\pst@onecoor{lineto}}%
  \def\rlineto{\pst@onecoor{rlineto}}%
  \def\curveto{\pst@threecoor{curveto}}%
  \def\rcurveto{\pst@threecoor{rcurveto}}%
  \def\code#1{\addto@pscode{#1}}%
  \def\coor(#1){\pst@@getcoor{#1}\addto@pscode\pst@coor\@ifnextchar({\coor}{}}%
  \def\rcoor{\pst@getcoors{}{}}%
  \def\dim#1{\pssetlength\pst@dimg{#1}\addto@pscode{\pst@number\pst@dimg}}%
  \def\setcolor#1{%
% ----------------hv begin 2004-05-07-------------------- patch 15
%  \@ifundefined{color@#1}{}{\addto@pscode{\use@color{#1}}}}%
%    \@ifundefined{color@#1}{}{\addto@pscode{\pst@usecolor{#1}}}}%
    \@ifundefined{\string\color@#1}{}{\addto@pscode{\pst@usecolor{#1}}}}%  hv 1.14  2005-12-17
% ----------------hv end 2004-05-07--------------------
  \def\arrows#1{{\psset@arrows{#1}\pst@addarrowdef}}%
  \let\file\pst@rawfile
} % END \pst@customdefs
\def\closedshadow@i{\cuse@par\pst@closedshadow}
\def\openshadow@i{\cuse@par\pst@openshadow}
\def\stroke@i{\cuse@par\pst@stroke}%
\def\fill@i{\cuse@par\psk@fillstyle}%
\def\pst@onecoor#1(#2){%
\pst@@getcoor{#2}%
\addto@pscode{\pst@coor #1}}
\def\pst@threecoor#1(#2)#3(#4)#5(#6){%
\begingroup
\pst@getcoor{#2}\pst@tempa
\pst@getcoor{#4}\pst@tempb
% DG/SR modification begin - Aug.  4, 1999 - Patch 11
%\pst@getcoor{#6}\pst@tembc
\pst@getcoor{#6}\pst@tempc
% DG/SR modification end
\addto@pscode{\pst@tempa \pst@tempb \pst@tempc #1}%
\endgroup}
\def\pst@rawfile#1{%
\begingroup
\def\do##1{\catcode`##1=12\relax}"
\dospecials
\catcode`\%=14
\pst@@rawfile{#1}%
\endgroup}
\def\pst@@rawfile#1{%
\immediate\openin1 #1
\ifeof1
\@pstrickserr{File `#1' not found}\@ehpa
\else
\immediate\read1 to \pst@tempg
\loop
\ifeof1 \@pstfalse\else\@psttrue\fi
\if@pst
\addto@pscode\pst@tempg
\immediate\read1 to \pst@tempg
\repeat
\fi
\immediate\closein1\relax}
\def\tx@NArray{NArray }
\def\tx@NArray{NArray }
\def\tx@Line{Line }
\def\tx@Arcto{Arcto }
\def\tx@CheckClosed{CheckClosed }
\def\tx@Polygon{Polygon }
\def\psset@gangle#1{\pst@getangle{#1}\psk@gangle}
\psset@gangle{0}
\def\tx@Diamond{Diamond }
\def\psdiamond{\pst@object{psdiamond}}
\def\psdiamond@i(#1){%
\@ifnextchar({\psdiamond@ii(#1)}{\psdiamond@ii(0,0)(#1)}}
\def\psdiamond@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@getcoor{#2}\pst@tempb
  \addto@pscode{%
    \psline@iii
    pop
    \psk@dimen
    \pst@tempb
    \psk@gangle
    \pst@tempa
    \tx@Diamond
  }%
  \def\pst@linetype{4}%
  \end@ClosedObj}
%
\def\tx@Triangle{Triangle }
\def\pstriangle{\pst@object{pstriangle}}
\def\pstriangle@i(#1){%
  \@ifnextchar({\pstriangle@ii(#1)}{\pstriangle@ii(0,0)(#1)}}
\def\pstriangle@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa%	the center of the baseline
  \pst@getcoor{#2}\pst@tempb%	the height of the triangle
  \addto@pscode{%
    \psline@iii
    pop			    %	no showpoints option
    \psk@dimen		    %	outer/inner/middle
    \pst@tempb
    \psk@gangle		    %	rotating angle
    \pst@tempa
    \tx@Triangle
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj}
%
\def\tx@CCA{CCA }
\def\tx@CCA{CCA }
\def\tx@CC{CC }
\def\tx@IC{IC }
\def\tx@BOC{BOC }
\def\tx@NC{NC }
\def\tx@EOC{EOC }
\def\tx@BAC{BAC }
\def\tx@NAC{NAC }
\def\tx@EAC{EAC }
\def\tx@OpenCurve{OpenCurve }
\def\tx@AltCurve{AltCurve }
\def\tx@ClosedCurve{ClosedCurve }
\def\psset@curvature#1{%
\edef\pst@tempg{#1 }%
\expandafter\psset@@curvature\pst@tempg * * * \@nil}
\def\psset@@curvature#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi
\edef\psk@curvature{\pst@tempg \pst@temph \pst@tempi}}
\psset@curvature{1 .1 0}
\def\pscurve{\pst@object{pscurve}}
\def\pscurve@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\pscurve@ii%
    }%
}
\def\pscurve@ii{%
  \addto@pscode{%
    \pst@cp
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \tx@OpenCurve%
  }%
  \end@OpenObj%
}
\def\psecurve{\pst@object{psecurve}}
\def\psecurve@i{%
\pst@getarrows{%
\begin@OpenObj
\pst@getcoors[\psecurve@ii}}
\def\psecurve@ii{%
\addto@pscode{%
\psk@curvature\space /c ED /b ED /a ED
\ifshowpoints true \else false \fi
\tx@AltCurve}%
\end@OpenObj}
\def\psccurve{\pst@object{psccurve}}
\def\psccurve@i{%
\begin@ClosedObj
\pst@getcoors[\psccurve@ii}
\def\psccurve@ii{%
\addto@pscode{%
\psk@curvature\space /c ED /b ED /a ED
\ifshowpoints true \else false \fi
\tx@ClosedCurve}%
\def\pst@linetype{1}%
\end@ClosedObj}
\def\psset@dotsize#1{%
\pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
\edef\psk@@dotsize{\pst@number\pst@dimg}%
\let\psk@@@dotsize\pst@tempg
\edef\psk@dotsize{%
  /DS \psk@@dotsize \psk@@@dotsize CLW mul add 2 div def }}
\psset@dotsize{2pt 2}
\def\psset@dotscale#1{%
\pst@getscale{#1}\psk@dotscale
\ifx\psk@dotscale\@empty
\def\psk@xdotscale{1 }%
\def\psk@ydotscale{1 }%
\else
\let\psk@xdotscale\pst@tempg
\let\psk@ydotscale\pst@temph
\fi}
% DG/SR modification begin - Oct. 17, 1997 - Patch 5
%\psset@dotscale{1}
% DG/SR modification end
\def\pst@Getangle#1#2{%
\pst@getangle{#1}\pst@tempg
\def\pst@temph{0. }%
\ifx\pst@tempg\pst@temph
\def#2{}%
\else
\edef#2{\pst@tempg\space rotate }%
\fi}
\def\psset@dotangle#1{%
\pst@getangle{#1}\psk@@dotangle
\ifdim\psk@@dotangle\p@=\z@
\let\psk@dotangle\@empty
\else
% DG/SR modification begin - Aug. 8, 1997 - Patch 4
%\edef\psk@dotangle{\psk@@dotangle rotate }
\edef\psk@dotangle{\psk@@dotangle rotate }%
% DG/SR modification end
\fi}
\psset@dotangle{0}
\def\pst@getdotsize{%
\pst@dimg=\psk@@@dotsize\pslinewidth
\advance\pst@dimg\psk@@dotsize\p@
\pst@dimh=\psk@ydotscale\pst@dimg
\pst@dimg=\psk@xdotscale\pst@dimg
\divide\pst@dimh 2
\divide\pst@dimg 2\relax}
% DG/SR modification begin - Oct. 17, 1997 - Patch 5
\psset@dotscale{1}
% DG/SR modification end
\def\psdot{\pst@object{psdot}}
\def\psdot@i{\@ifnextchar({\psdot@ii}{\psdot@ii(\z@,\z@)}}
\def\psdot@ii(#1){%
  \begin@SpecialObj
% hv modification 1.13 2005-11-28 
  \solid@star
% hv modification end 
  \pst@@getcoor{#1}%
  \addto@pscode{%
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}%
    \pst@coor Dot}%
  \end@SpecialObj}
\def\psdots{\pst@object{psdots}}
\def\psdots@i{%
  \begin@SpecialObj
  \pst@getcoors[\psdots@ii}
\def\psdots@ii{%
  \addto@pscode{false \tx@NArray \psdots@iii}%
  \end@SpecialObj}
\def\psdots@iii{%
  \psk@dotsize
  \@nameuse{psds@\psk@dotstyle}
  newpath
  n { transform floor .5 add exch floor .5 add exch itransform Dot } repeat}
%
% DG: dead code (to suppress until \psset@dotstyle) ? - Aug. 4, 1997
\def\tx@SQ{SQ }
\def\tx@ST{ST }
\def\tx@SP{SP }
%
\def\pst@gdot#1{/Dot { gsave T \psk@dotangle \psk@dotscale #1 grestore } def }
%
\@namedef{psds@*}{\pst@gdot{0 0 DS \tx@SD}}
\@namedef{psds@o}{%
  /r2 DS CLW sub def
  \pst@gdot{0 0 DS \tx@SD \pst@usecolor\psfillcolor 0 0 r2 \tx@SD}}
\@namedef{psds@square*}{%
  /r1 DS .886 mul def
  \pst@gdot{r1 \tx@SQ}}
\@namedef{psds@square}{%
  /r1 DS .886 mul def /r2 r1 CLW sub def
  \pst@gdot{r1 \tx@SQ \pst@usecolor\psfillcolor r2 \tx@SQ}}
\@namedef{psds@triangle*}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST}}
\@namedef{psds@triangle}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  /y2 y1 CLW add def /x2 y2 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST \pst@usecolor\psfillcolor x2 y2 \tx@ST}}
\@namedef{psds@pentagon*}{%
  /r1 DS 1.149 mul def
  \pst@gdot{r1 \tx@SP}}
\@namedef{psds@pentagon}{%
  DS .93 mul dup 1.236 mul /r1 ED CLW sub 1.236 mul /r2 ED
  \pst@gdot{r1 \tx@SP \pst@usecolor\psfillcolor r2 \tx@SP}}
\@namedef{psds@+}{%
  /DS DS 1.253 mul def
  \pst@gdot{DS 0 moveto DS neg 0 L stroke 0 DS moveto 0 DS neg L stroke}}
\@namedef{psds@|}{%
  \psk@tbarsize CLW mul add 2 div /DS ED
  \pst@gdot{0 DS moveto 0 DS neg L stroke}}
% DG: end dead code?
%
\def\psset@dotstyle#1{%
\@ifundefined{psds@#1}%
{\@pstrickserr{Dot style `#1' not defined}\@eha}%
{\edef\psk@dotstyle{#1}}}
\psset@dotstyle{*}
%
\def\tx@FontDot{FontDot }
\def\newpsfontdot#1[#2]#3#4{%
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
% DG/SR modification begin - Dec. 12, 1999 - Patch 14
%/Dot { moveto #4 show } bind def }}
    /Dot { moveto gsave \psk@dotscale #4 show grestore } bind def 
}}
% DG/SR modification end
\def\newpsfontdotH#1[#2]#3#4#5{%
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
    /Dot {
      moveto
      \iftrue
% DG/SR modification begin - Dec. 23, 1999 - Patch 14
%gsave \pst@usecolor\psfillcolor #5 show grestore
%\fi
%#4 show
      gsave \psk@dotscale \pst@usecolor\psfillcolor #5 show grestore
      \fi
      gsave \psk@dotscale #4 show grestore
% DG/SR modification end
    } bind def 
}}
%
\pstheader{pst-dots.pro}
\newpsfontdot{*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{o}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{Bo}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
\newpsfontdotH{triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{Btriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{triangle*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{Bsquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{square*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdotH{pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{Bpentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{pentagon*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
% DG/SR modification begin - Mar. 18, 1997 and Dec. 16, 1999 - Patch 14
%\newpsfontdot{diamond*}%
%[1.9 0.0 0.0 1.9 -0.4598 -0.70775]{Symbol}{<E0>}
%\newpsfontdot{diamond}%
%[2.3 0.0 0.0 2.3 -0.8533 -0.5336]{Symbol}{<A8>}
% D.G. modification begin - Jan. 17, 2000
\newpsfontdotH{diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{Bdiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{diamond*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
% DG/SR modification end
\newpsfontdot{oplus}[1.44928 0.0 0.0 1.44928 -0.562319 -0.478261]{Symbol}{<C5>}
\newpsfontdot{otimes}[1.44928 0.0 0.0 1.44928 -0.562319 -0.475362]{Symbol}{<C4>}
\newpsfontdot{x}[1.8 0.0 0.0 1.8 -0.495 -0.4788]{Symbol}{<B4>}
\newpsfontdot{+}[2.3 0.0 0.0 2.3 -0.6486 -0.5819]{Times-Roman}{<2B>}
\newpsfontdot{asterisk}[2.43309 0.0 0.0 2.43309 -0.609489 -1.14477]{Times-Roman}{<2A>}
\newpsfontdot{B+}[2.3 0.0 0.0 2.3 -0.6555 -0.5819]{Times-Bold}{<2B>}
\newpsfontdot{Basterisk}[2.29358 0.0 0.0 2.29358 -0.576835 -1.08486]{Times-Bold}{<2A>}
\newpsfontdot{|}[1.98413 0.0 0.0 1.38 -0.258929 -0.5]{Helvetica}{(|)}
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.258929 -0.712302]{Helvetica}{(|)}
% DG/SR modification end
\newpsfontdot{B|}[1.98413 0.0 0.0 1.38 -0.277778 -0.5]{Helvetica-Bold}{(|)}%
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.277778 -0.78302]{Helvetica-Bold}{(|)}

% DG/SR modification end
\iffalse
\newpsfontdot{*}[2.77778 0.0 0.0 2.77778 -0.638889 -0.813889]{Symbol}{<B7>}
\newpsfontdot{o}[3.33333 0.0 0.0 3.33333 -0.666667 -1.78167]{Symbol}{<B0>}
\newpsfontdot{Bo}[4.69484 0.0 0.0 4.69484 -0.78169 -2.97418]{Times-Bold}{<CA>}
\fi
% Etienne Riga
\newpsfontdot{Asterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(k)}
\newpsfontdot{BoldAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(K)}
\newpsfontdotH{SolidAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(J)}{(b)}
\newpsfontdotH{Hexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(h)}{(G)}
\newpsfontdotH{BoldHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(H)}{(G)}
\newpsfontdot{SolidHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(G)}
%
\newpsfontdot{Bullet}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{Circle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{BoldCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
%\newpsfontdot{SolidCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{BoldTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{SolidTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{BoldSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{SolidSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdotH{Pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{BoldPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{SolidPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
\newpsfontdot{Add}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(a)}
\newpsfontdot{BoldAdd}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(A)}
\newpsfontdot{Mul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(x)}
\newpsfontdot{BoldMul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(X)}
\newpsfontdotH{Oplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(m)}{(b)}
\newpsfontdotH{BoldOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(M)}{(b)}
\newpsfontdotH{SolidOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(e)}{(b)}
\newpsfontdotH{Otimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(n)}{(b)}
\newpsfontdotH{BoldOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(N)}{(b)}
\newpsfontdotH{SolidOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(E)}{(b)}
\newpsfontdot{Bar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(i)}
\newpsfontdot{BoldBar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(I)}
\newpsfontdotH{Diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{BoldDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{SolidDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
%%
\newdimen\pslinearc
\def\psset@linearc#1{\pssetlength\pslinearc{#1}}
\psset@linearc{0pt}
\def\psline{\pst@object{psline}}
\def\psline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psline@ii%
  }%
}
\def\psline@ii{%
  \addto@pscode{\pst@cp \psline@iii \tx@Line}%
  \end@OpenObj%
}
\def\psline@iii{%
  \ifdim\pslinearc>\z@
    /r \pst@number\pslinearc def
    /Lineto { \tx@Arcto } def
  \else
    /Lineto /lineto load def
  \fi
  \ifshowpoints true \else false \fi
}
\def\qline(#1)(#2){%
  \def\pst@par{}%
  \begin@SpecialObj
  \def\pst@linetype{0}%
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{%
    \pst@tempa moveto \pst@coor L
    \@nameuse{psls@\pslinestyle}%
  }%
  \end@SpecialObj}
\def\pspolygon{\pst@object{pspolygon}}
\def\pspolygon@i{%
  \begin@ClosedObj%
  \def\pst@cp{}%
  \pst@getcoors[\pspolygon@ii%
}
\def\pspolygon@ii{%
  \addto@pscode{\psline@iii \tx@Polygon}%
  \def\pst@linetype{1}%
  \end@ClosedObj%
}
\def\psset@framearc#1{\pst@checknum{#1}\psk@framearc}
\psset@framearc{0}
\def\psset@cornersize#1{%
\pst@expandafter\psset@@cornersize{#1}\@nil}
\def\psset@@cornersize#1#2\@nil{%
\if #1a\relax
\def\psk@cornersize{\pst@number\pslinearc false }%
\else
\def\psk@cornersize{\psk@framearc true }%
\fi}
\psset@cornersize{relative}
\def\tx@Rect{Rect }
\def\tx@OvalFrame{OvalFrame }
\def\tx@Frame{Frame }
%
\def\psset@dimen#1{\pst@expandafter\psset@@dimen{#1}\@nil}
\def\psset@@dimen#1#2\@nil{%
  \if #1o\relax%	outer
    \def\psk@dimen{.5 }%
  \else
    \if #1m\relax%	middle
      \def\psk@dimen{0 }%
    \else
      \if #1i\relax%	inner
        \def\psk@dimen{-.5 }%
  \fi\fi\fi}
\psset@dimen{outer}
%
\def\psframe{\pst@object{psframe}}
\def\psframe@i(#1){%
  \@ifnextchar({\psframe@ii(#1)}{\psframe@ii(0,0)(#1)}}
\def\psframe@ii(#1)(#2){%
  \begin@ClosedObj
    \pst@getcoor{#1}\pst@tempa
    \pst@@getcoor{#2}%
    \addto@pscode{\psk@cornersize \pst@tempa \pst@coor \psk@dimen \tx@Frame}%
    \def\pst@linetype{2}%
    \showpointsfalse
  \end@ClosedObj%
}
\def\tx@BezierNArray{BezierNArray }
\def\tx@OpenBezier{OpenBezier }
\def\tx@ClosedBezier{ClosedBezier }
\def\tx@BezierShowPoints{BezierShowPoints }
\def\psbezier{\pst@object{psbezier}}
\def\psbezier@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\psbezier@ii%
  }%
}
\def\psbezier@ii{%
  \addto@pscode{%
% DG/SR modification begin - Apr. 28, 1997 - Patch 1
% \psbezier doesn't work inside \pscustom
\pst@cp
% DG/SR modification end
    \ifshowpoints true \else false \fi
    \tx@OpenBezier
    \ifshowpoints \tx@BezierShowPoints \fi}%
  \end@OpenObj}
\def\pscbezier{\pst@object{pscbezier}}
\def\pscbezier@i{%
  \begin@ClosedObj
  \pst@getcoors[\pscbezier@ii}
\def\pscbezier@ii{%
  \addto@pscode{%
    \ifshowpoints true \else false \fi
    \tx@ClosedBezier
    \ifshowpoints \tx@BezierShowPoints \fi}%
  \chardef\pst@linetype=1
  \end@ClosedObj}
\def\tx@Parab{Parab }
\def\parabola{\pst@object{parabola}}
\def\parabola@i{\pst@getarrows\parabola@ii}
\def\parabola@ii#1(#2)#3(#4){%
\begin@OpenObj
\pst@getcoor{#2}\pst@tempa
\pst@@getcoor{#4}%
\addto@pscode{\pst@tempa \pst@coor \tx@Parab}%
\end@OpenObj}
%
\def\psset@gridwidth#1{\pst@getlength{#1}\psk@gridwidth}
\psset@gridwidth{.8pt}
\def\psset@griddots#1{%
  \pst@cntg=#1\relax
  \edef\psk@griddots{\the\pst@cntg}}
\psset@griddots{0}
\def\psset@gridcolor#1{\pst@getcolor{#1}\psgridcolor}
\psset@gridcolor{black}
\def\psset@subgridwidth#1{\pst@getlength{#1}\psk@subgridwidth}
\psset@subgridwidth{.4pt}
\def\psset@subgridcolor#1{\pst@getcolor{#1}\pssubgridcolor}
\psset@subgridcolor{gray}
\def\psset@subgriddots#1{%
  \pst@cntg=#1\relax\edef\psk@subgriddots{\the\pst@cntg}}
\psset@subgriddots{0}
\def\psset@subgriddiv#1{%
  \pst@cntg=#1\relax\edef\psk@subgriddiv{\the\pst@cntg}}
\psset@subgriddiv{5}
\def\psset@gridlabels#1{\pst@getlength{#1}\psk@gridlabels}
\psset@gridlabels{10pt}
\def\psset@gridlabelcolor#1{\pst@getcolor{#1}\psgridlabelcolor}
\psset@gridlabelcolor{black}
\def\tx@Grid{Grid }
\def\psgrid{\pst@object{psgrid}}
\def\psgrid@i{\@ifnextchar(%
  {\psgrid@ii}{\expandafter\psgrid@iv\pic@coor}}
\def\psgrid@ii(#1){\@ifnextchar(%
  {\psgrid@iii(#1)}{\psgrid@iv(0,0)(0,0)(#1)}}
\def\psgrid@iii(#1)(#2){\@ifnextchar(%
  {\psgrid@iv(#1)(#2)}{\psgrid@iv(#1)(#1)(#2)}}
\def\psgrid@iv(#1)(#2)(#3){%
  \begin@SpecialObj
    \pst@getcoor{#1}\pst@tempA%  hv 1.11
    \pst@getcoor{#2}\pst@tempB % hv 1.11
    \pst@@getcoor{#3}%
    \ifnum\psk@subgriddiv>1
      \addto@pscode{
        gsave
        \psk@subgridwidth SLW \pst@usecolor\pssubgridcolor
        \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
%        \pst@number\psxunit \pst@number\psyunit        % hv 1.11
        \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
        \psk@subgriddiv\space \psk@subgriddots\space
        {} 0 \tx@Grid 
	grestore
      }%
    \fi
    \addto@pscode{%
      gsave
      \psk@gridwidth SLW \pst@usecolor\psgridcolor
      \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
      \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
%      \pst@number\psxunit \pst@number\psyunit        % hv 1.11
      1 \psk@griddots\space { \pst@usecolor\psgridlabelcolor }
      \psk@gridlabels \tx@Grid 
      grestore
    }%
  \end@SpecialObj%
}
%
\newif\ifpsmathbox
\psmathboxtrue
\def\pst@mathflag{\z@}
\newtoks\everypsbox
\let\pst@thisbox\relax
\long\def\pst@makenotverbbox#1#2{%
  \edef\pst@mathflag{%
  \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi}%
  \setbox\pst@hbox=\hbox{%
    \ifcase\pst@mathflag\or$\m@th\textstyle\or$\m@th\displaystyle\fi
    {\pst@thisbox\the\everypsbox#2}%
    \ifnum\pst@mathflag>\z@$\fi% $
  }%
  #1%
}
\def\pst@makeverbbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{%
    \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi%
  }%
  \afterassignment\pst@beginbox
  \setbox\pst@hbox\hbox%
}
\def\pst@beginbox{%
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
  \bgroup\aftergroup\pst@endbox
  \pst@thisbox
  \the\everypsbox%
}
\def\pst@endbox{%
  \ifnum\pst@mathflag>\z@$\fi
  \egroup
  \pst@afterbox%
}
\def\pst@makebox{\pst@@makebox}
\def\psverbboxtrue{\def\pst@@makebox{\pst@makeverbbox}}
\def\psverbboxfalse{\def\pst@@makebox{\pst@makenotverbbox}}
\psverbboxfalse
\def\pst@longbox{%
  \def\pst@makebox{%
    \gdef\pst@makebox{\pst@@makebox}%
    \pst@makelongbox%
  }%
}
\def\pst@makelongbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{%
    \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi%
  }%
  \setbox\pst@hbox\hbox\bgroup
  \aftergroup\pst@afterbox
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
  \begingroup
  \pst@thisbox
  \the\everypsbox%
}
\def\pst@endlongbox{%
  \endgroup
  \ifnum\pst@mathflag>\z@$\fi
  \egroup%
}
\def\pslongbox#1#2{%
\@namedef{#1}{\pst@longbox#2}%
\@namedef{end#1}{\pst@endlongbox}%
}
\newdimen\psframesep
\def\psset@framesep#1{\pssetlength\psframesep{#1}}
\psset@framesep{3pt}
\newif\ifpsboxsep
\def\psset@boxsep#1{\@nameuse{psboxsep#1}}
\psset@boxsep{true}
\def\pst@useboxpar{%
  \use@par
  \if@star
    \let\pslinecolor\psfillcolor
    \solid@star
    \let\solid@star\relax
  \fi
  \ifpsdoubleline \pst@setdoublesep \fi%
}
\def\psframebox{\pst@object{psframebox}}
\def\psframebox@i{\pst@makebox\psframebox@ii}
\def\psframebox@ii{%
  \begingroup
  \pst@useboxpar
  \pst@dima=\pslinewidth
  \advance\pst@dima by \psframesep
  \pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
  \pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
  \setbox\pst@hbox=\hbox{%
    \ifpsboxsep\kern\pst@dima\fi
    \begin@ClosedObj
    \addto@pscode{%
      \psk@cornersize
      \pst@number\pst@dima neg
      \pst@number\pst@dimb neg
      \pst@number\pst@dimc
      \pst@number\pst@dimd
      .5
      \tx@Frame%
    }%
    \def\pst@linetype{2}%
    \showpointsfalse
    \end@ClosedObj
    \box\pst@hbox
    \ifpsboxsep\kern\pst@dima\fi%
  }%
  \ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
  \leavevmode\box\pst@hbox
  \endgroup%
}
\def\psdblframebox{\pst@object{psdblframebox}}
\def\psdblframebox@i{\addto@par{doubleline=true}\psframebox@i}
\def\psclip#1{%
  \leavevmode
  \begingroup
    \begin@psclip
      \begingroup
        \def\use@pscode{%
          \pstVerb{%
            \pst@dict
            /mtrxc CM def
            CP CP T
            \tx@STV
            \psk@origin
            \psk@swapaxes
            newpath
            \pst@code
            clip
            newpath
            mtrxc setmatrix
            moveto
            0 setgray
            end
	  }%
          \gdef\pst@code{}}%
  \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
  \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
  \hbox to\z@{#1}%
  \endgroup
  \def\endpsclip{%
    \end@psclip
    \endgroup}%
  \ignorespaces}
\def\endpsclip{\pst@misplaced\endpsclip}
\let\begin@psclip\relax
\def\end@psclip{\pstVerb{currentpoint initclip moveto}}
\def\AltClipMode{%
\def\end@psclip{\pstVerb{\pst@grestore}}%
\def\begin@psclip{\pstVerb{gsave}}}
\def\clipbox{\@ifnextchar[{\clipbox@}{\clipbox@[\z@]}}
% DG modification begin - Apr. 3, 1997
% From paulus@immd5.informatik.uni-erlangen.de (Dietrich Paulus)
%\def\clipbox@[#1]{\pst@makebox\clipbox@@{#1}}
\def\clipbox@[#1]{\pst@makebox{\clipbox@@{#1}}}
% DG modification end
\def\clipbox@@#1{%
  \pssetlength\pst@dimg{#1}%
  \leavevmode\hbox{%
  \begin@psclip
  \pst@Verb{%
    CM \tx@STV CP T newpath
    /a \pst@number\pst@dimg def
    /w \pst@number{\wd\pst@hbox}a add def
    /d \pst@number{\dp\pst@hbox}a add neg def
    /h \pst@number{\ht\pst@hbox}a add def
    a neg d moveto
    a neg h L
    w h L
    w d L
    closepath
    clip
    newpath
    0 0 moveto
    setmatrix}%
\unhbox\pst@hbox
\end@psclip}}
\def\psshadowbox{\pst@object{psshadowbox}}
\def\psshadowbox@i{\pst@makebox\psshadowbox@ii}
\def\psshadowbox@ii{%
\begingroup
\pst@useboxpar
\psshadowtrue
\psboxseptrue
\def\psk@shadowangle{-45 }%
\setbox\pst@hbox=\hbox{\psframebox@ii}%
\pst@dimh=\psk@shadowsize\p@
\pst@dimh=.7071\pst@dimh
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pst@dimh
\dp\pst@hbox=\pst@dimg
\pst@dimg=\wd\pst@hbox
\advance\pst@dimg\pst@dimh
\wd\pst@hbox=\pst@dimg
\leavevmode
\box\pst@hbox
\endgroup}
\def\pscirclebox{\pst@object{pscirclebox}}
\def\pscirclebox@i{\pst@makebox\pscirclebox@ii}
\def\pscirclebox@ii{%
\begingroup
\pst@useboxpar
\setbox\pst@hbox=\hbox{%
\pst@nodehook
\pscirclebox@iii
\box\pst@hbox}%
\ifpsboxsep \pscirclebox@sep \fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\pscirclebox@iii{%
\if@star
\pslinewidth\z@
\pstverb{\pst@dict \tx@STP \pst@usecolor\psfillcolor
newpath \pscirclebox@iv \tx@SD end}%
\else
\begin@ClosedObj
\def\pst@linetype{4}\showpointsfalse
\addto@pscode{%
\pscirclebox@iv CLW 2 div add 0 360 arc closepath}%
\end@ClosedObj
\fi}
\def\pscirclebox@iv{%
\pst@number{\wd\pst@hbox}2 div
\pst@number{\ht\pst@hbox}\pst@number{\dp\pst@hbox}add 2 div
2 copy \pst@number{\dp\pst@hbox}sub 4 2 roll
\tx@Pyth \pst@number\psframesep add }
\def\pscirclebox@sep{%
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\dp\pst@hbox
\divide\pst@dimb 2
\pst@dima=.5\wd\pst@hbox
\pst@pyth\pst@dima\pst@dimb\pst@dimc
\advance\pst@dimc\pslinewidth
\advance\pst@dimc\psframesep
\advance\pst@dimb-\pst@dimc
\setbox\pst@hbox=\hbox to2\pst@dimc{%
\hss
\vbox{\kern-\pst@dimb\box\pst@hbox}%
\hss}%
\advance\pst@dimb-\dp\pst@hbox
\dp\pst@hbox=-\pst@dimb}
\let\pst@nodehook\relax
\def\psCirclebox{\pst@object{psCirclebox}}
\def\psCirclebox@i{\pst@makebox\psCirclebox@ii}
\def\psCirclebox@ii{%
\begingroup
\pst@useboxpar
\pst@dima=\ht\pst@hbox
\advance\pst@dima\dp\pst@hbox
\divide\pst@dima\tw@
\pssetlength\pst@dimb\psk@radius
\setbox\pst@hbox=\hbox{%
\pst@nodehook
\pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
\box\pst@hbox}%
\ifpsboxsep \psCirclebox@sep \fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psCirclebox@sep{%
\pst@dimc=\pst@dimb
\advance\pst@dimb-\pst@dima
\advance\pst@dima\pst@dimc
\setbox\pst@hbox=\hbox to\tw@\pst@dimc{%
\hss
\vrule width \z@ depth \pst@dimb height \pst@dima
\box\pst@hbox
\hss}}%
\def\psovalbox{\pst@object{psovalbox}}
\def\psovalbox@i{\pst@makebox{\psovalbox@ii}}
\def\psovalbox@ii{%
\begingroup
\pst@useboxpar
\psovalbox@iii
\ifpsboxsep\psovalbox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psovalbox@iii{%
\psovalbox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
0 360
\pst@number\pst@dimc CLW 2 div sub
\pst@number\pst@dimd CLW 2 div sub
\pst@number\pst@dima
\pst@number\pst@dimb
\tx@Ellipse
closepath}%
\def\pst@linetype{2}%
\end@ClosedObj
\unhbox\pst@hbox}}
\def\psovalbox@iv{%
\pst@dimc=\pslinewidth\advance\pst@dimc\psframesep
\pst@dimd=\ht\pst@hbox\advance\pst@dimd\dp\pst@hbox
\pst@dima=.5\wd\pst@hbox
\pst@dimb=.5\pst@dimd\advance\pst@dimb-\dp\pst@hbox
\pst@dimd=.707\pst@dimd
\advance\pst@dimd\pst@dimc
\advance\pst@dimc.707\wd\pst@hbox}
\def\psovalbox@sep{%
\setbox\pst@hbox\hbox to 2\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\pst@dimg=\pst@dimd
\advance\pst@dimg-\pst@dimb
\dp\pst@hbox=\pst@dimg
\advance\pst@dimd\pst@dimb
\ht\pst@hbox=\pst@dimd}
\def\psdiabox{\pst@object{psdiabox}}
\def\psdiabox@i{\pst@makebox{\psdiabox@ii}}
\def\psdiabox@ii{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\ifpsboxsep\psdiabox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psdiabox@iv{%
\pst@dimg=.707\pslinewidth
\advance\pst@dimg.707\psframesep
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimc=\pst@dima
\advance\pst@dimc\pst@dimg
\pst@dimd=\ht\pst@hbox
\advance\pst@dimd\dp\pst@hbox
\divide\pst@dimd 2
\pst@dimb=\pst@dimd
\advance\pst@dimb-\dp\pst@hbox
\advance\pst@dimd\pst@dimg}
\def\psdiabox@iii{%
\psdiabox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc 2 mul \pst@number\pst@dimd 2 mul
0
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Diamond}%
\def\pst@linetype{4}%
\end@ClosedObj
\box\pst@hbox}}
\def\psdiabox@sep{%
\setbox\pst@hbox\hbox to 4\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\multiply\pst@dimd 2
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\advance\pst@dimd-2\pst@dimb
\dp\pst@hbox\pst@dimd}
\def\psset@trimode#1{\pst@expandafter\psset@@trimode{#1}\@empty\@empty\@nil}
\def\psset@@trimode#1#2#3\@nil{%
\let\pst@tempg#1\relax
\ifx\pst@tempg*%
\let\psk@@trimode\@empty
\let\pst@tempg#2\relax
\else
\let\psk@@trimode\relax
\fi
\edef\psk@trimode{%
\ifx R\pst@tempg 1 \else\ifx D\pst@tempg 2
\else\ifx L\pst@tempg 3 \else 0 \fi\fi\fi}}
\psset@trimode{U}
\def\pstribox{\pst@object{pstribox}}
\def\pstribox@i{\pst@makebox{\pstribox@ii}}
\def\pstribox@ii{%
\begingroup
\pst@useboxpar
\pstribox@iii
\ifpsboxsep\pstribox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\pstribox@iii{%
\pstribox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc \pst@number\pst@dimd
\ifodd\psk@trimode exch \fi
\psk@trimode -90 mul
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Triangle}%
\def\pst@linetype{2}%
\end@ClosedObj
\box\pst@hbox}}
\def\pstribox@iv{%
\pst@dimh=\pslinewidth
\advance\pst@dimh\psframesep
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg-\dp\pst@hbox
\divide\pst@dimg 2
\edef\pst@tempa{\number\pst@dimg sp}% For use by nodes.
\ifodd\psk@trimode
\pst@dimb\pst@dimg
\else
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\fi
\ifcase\psk@trimode
\pst@dimb=-\dp\pst@hbox
\advance\pst@dimb-\pst@dimh
\or
\pst@dima=-\pst@dimh
\or
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\pst@dimh
\or
\pst@dima=\wd\pst@hbox
\advance\pst@dima\pst@dimh
\fi
\pst@dimd=\dp\pst@hbox
\advance\pst@dimd\ht\pst@hbox
\ifx\psk@@trimode\relax
\pst@dimc=\wd\pst@hbox
\advance\pst@dimc\ifodd\psk@trimode 1.447\else 1.789\fi\pst@dimh
\multiply\pst@dimc 2
\advance\pst@dimd\ifodd\psk@trimode 1.789\else 1.447\fi\pst@dimh
\multiply\pst@dimd 2
\else
\ifodd\psk@trimode
\advance\pst@dimd 1.1547\wd\pst@hbox
\advance\pst@dimd 3.4641\pst@dimh
\pst@dimc=.866\pst@dimd
\else
\advance\pst@dimd .866\wd\pst@hbox %.866=(sqrt(3)/2)
\advance\pst@dimd 3\pst@dimh
\pst@dimc=1.1547\pst@dimd % 1.1547=(2/sqrt(3))
\fi
\fi}
\def\pstribox@sep{%
\ifodd\psk@trimode
\advance\pst@dimb.5\pst@dimd
\ht\pst@hbox=\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox=\pst@dimd
\else
\setbox\pst@hbox\hbox to \pst@dimc{\hss\unhbox\pst@hbox\hss}%
\global\pst@dimg=.5\pst@dimc
\fi
\ifcase\psk@trimode
\dp\pst@hbox-\pst@dimb
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\or
\pst@dimg=.5\wd\pst@hbox
\global\advance\pst@dimg-\pst@dima
\setbox\pst@hbox\hbox to \pst@dimc{\kern-\pst@dima\box\pst@hbox\hss}%
\or
\ht\pst@hbox\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox\pst@dimd
\or
\pst@dimg=\pst@dimc
\advance\pst@dimg-\pst@dima
\global\advance\pst@dimg.5\wd\pst@hbox
\setbox\pst@hbox\hbox to \pst@dimc{%
\hss\box\pst@hbox\kern\psframesep\kern\pslinewidth}%
\fi}
\def\psset@arcsepA#1{\pst@getlength{#1}\psk@arcsepA}
\def\psset@arcsepB#1{\pst@getlength{#1}\psk@arcsepB}
\def\psset@arcsep#1{%
\psset@arcsepA{#1}\let\psk@arcsepB\psk@arcsepA}
\psset@arcsep{0}
\def\tx@ArcArrow{ArcArrow }
\def\psarc{\pst@object{psarc}}
\def\psarc@i{\@ifnextchar({\psarc@iii}{\psarc@ii}}
\def\psarc@ii#1{\addto@par{arrows=#1}%
  \@ifnextchar({\psarc@iii}{\psarc@iii(0,0)}%
}
\def\psarc@iii(#1)#2#3#4{%
  \begin@OpenObj
    \pst@getangle{#3}\pst@tempa
    \pst@getangle{#4}\pst@tempb
    \pst@@getcoor{#1}%
    \pssetlength\pst@dima{#2}%
    \addto@pscode{\psarc@iv \psarc@v}%
    \gdef\psarc@type{0}%
    \showpointsfalse
  \end@OpenObj%
}
\def\psarc@iv{%
  \pst@coor /y ED /x ED
  /r \pst@number\pst@dima def
  /c 57.2957 r \tx@Div def
  /angleA
    \pst@tempa
    \psk@arcsepA c mul 2 div
    \ifcase \psarc@type add \or sub \fi
  def
  /angleB
    \pst@tempb
    \psk@arcsepB c mul 2 div
    \ifcase \psarc@type sub \or add \fi
  def
  \ifshowpoints\psarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      r angleA \tx@PtoC
      y add exch x add exch moveto
    \fi
  \fi}
% hv ---- 1.10 2005-05-05 ----------------------> hv begin
\def\psarc@v{%
  x y r
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    r 0 gt \pslbrace
    { \ifcase\psarc@type add \or sub \fi } \psrbrace\pslbrace
    { \ifcase\psarc@type sub \or add \fi } \psrbrace ifelse
%    { \ifcase\psarc@type add \or sub \fi }
    \tx@ArcArrow
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    r 0 gt \pslbrace
      { \ifcase\psarc@type sub \or add \fi } \psrbrace\pslbrace
      { \ifcase\psarc@type add \or sub \fi } \psrbrace ifelse
%      { \ifcase\psarc@type sub \or add \fi }
 \tx@ArcArrow
  \fi
\ifcase\psarc@type arc \or arcn \fi}
% hv ----- 1.10 2005-05-05 ------------------------> end
%
\def\psarc@type{0}
\def\psarc@showpoints{%
  gsave
  newpath
  x y moveto
  x y r \pst@tempa \pst@tempb
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash stroke
  grestore }
\def\psarcn{\pst@object{psarcn}}
\def\psarcn@i{\def\psarc@type{1}\psarc@i}
%
%------------------ tvz/DG/hv (2004-05-10) begin -------------------%%
% from Denis Giroux: http://www.tug.org/pipermail/pstricks/2001/000507.html
%
% I - Definition of \psellipticwedge, a generalization of \pswedge for wedges
%     of ellipses (from the code of \pswedge and \psellipse)
%
\def\psellipticwedge{\def\pst@par{}\pst@object{psellipticwedge}}
\def\psellipticwedge@i(#1){%
  \@ifnextchar({\psellipticwedge@ii(#1)}{\psellipticwedge@ii(0,0)(#1)}}
\def\psellipticwedge@ii(#1)(#2)#3#4{%
  \begin@ClosedObj
    \pst@getangle{#3}\pst@tempa
    \pst@getangle{#4}\pst@tempb
    \pst@getcoor{#1}\pst@tempc
    \pst@@getcoor{#2}%
    \def\pst@linetype{1}%
    \addto@pscode{%
      \pst@tempa \pst@tempb
      \pst@coor
      \pst@tempc moveto
      \ifdim\psk@dimen\p@=\z@\else
        \psk@dimen CLW mul dup 3 1 roll
        sub 3 1 roll sub exch
      \fi
      \pst@tempc
      \tx@Ellipse
      closepath%
    }%
    \showpointsfalse
  \end@ClosedObj%
}
%
% Code mainly from "pstricks.tex'' 0.94 beta (TvZ)
%
\def\psellipticarcn{\def\pst@par{}\pst@object{psellipticarcn}}
\def\psellipticarcn@i{\let\if@psarcn\iftrue\psellipticarc@ii}
%
\def\psellipticarc{\def\pst@par{}\pst@object{psellipticarc}}
\def\psellipticarc@i{\let\if@psarcn\iffalse\psellipticarc@ii}
%
\let\if@psarcn\iffalse
\def\psellipticarc@ii{\pst@getarrows\psellipticarc@iii}
\def\psellipticarc@iii(#1){%
	\@ifnextchar({\psellipticarc@iv(#1)}{\psellipticarc@iv(0,0)(#1)}}
\def\psellipticarc@iv(#1)(#2)#3#4{%
  \begin@OpenObj
  \pst@getcoor{#1}\pst@tempa
  \pst@getcoor{#2}\pst@tempb
  \pst@getangle{#3}\pst@tempc
  \pst@getangle{#4}\pst@tempd
  \addto@pscode{\psellipticarc@definearg \psellipticarc@draw}%
  \showpointsfalse
  \end@OpenObj%
}
\def\psellipticarc@definearg{%
  \pst@tempa /y ED /x ED  % Origin
  \pst@tempb              % radii. Now adjust:
  \ifdim\psk@dimen\p@=\z@\else
    \psk@dimen CLW mul dup 3 1 roll
    sub 3 1 roll sub exch
  \fi
  /ry ED /rx ED
  /angleA
    /d {  \if@psarcn sub \else add \fi } def
    \pst@tempc \psk@arcsepA 2 div
    ArcAdjust
  def
  /angleB
    /d  {  \if@psarcn add \else sub \fi } def
      \pst@tempd \psk@arcsepB 2 div
      ArcAdjust
    def
    \ifshowpoints\psellipticarc@showpoints\fi
    \ifx\psk@arrowA\@empty
      \ifnum\psk@liftpen=2
	angleA cos rx mul x add
	angleA sin ry mul y add
	moveto
     \fi
   \fi%
}
\def\psellipticarc@draw{%
  0 0 1
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    { \if@psarcn sub \else add \fi }
    EllipticArcArrow
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    { \if@psarcn add \else sub \fi }
    EllipticArcArrow
  \fi
  /mtrx CM def
  x y T
  rx ry scale
  \if@psarcn arcn \else arc \fi
  mtrx setmatrix%
}
\def\psellipticarc@showpoints{%
  gsave
  /mtrx CM def
  x y T
  rx ry scale
  0 0 moveto
  0 0 1 \pst@tempc \pst@tempd
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  mtrx setmatrix
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash stroke
  grestore %
}
\def\pscircle{\pst@object{pscircle}}
\def\pscircle@i{\@ifnextchar({\pscircle@do}{\pscircle@do(0,0)}}
\def\pscircle@do(#1)#2{%
\if@star
{\use@par\qdisk(#1){#2}}%
\else
\begin@ClosedObj
\pst@@getcoor{#1}%
\pssetlength\pst@dimc{#2}%
\def\pst@linetype{4}%
\addto@pscode{%
\pst@coor
\pst@number\pst@dimc
\psk@dimen CLW mul sub
0 360 arc
closepath}%
\showpointsfalse
\end@ClosedObj
\fi
\ignorespaces}
\def\qdisk(#1)#2{%
\def\pst@par{}%
\begin@SpecialObj
\pst@@getcoor{#1}%
\pssetlength\pst@dimg{#2}%
\addto@pscode{\pst@coor \pst@number\pst@dimg \tx@SD}%
\end@SpecialObj}
\def\psset@radius#1{\pst@@getlength{#1}\psk@radius}
\psset@radius{.25cm}
\def\psCircle{\pst@object{psCircle}}
\def\psCircle@i{\@ifnextchar({\psCircle@ii}{\psCircle@ii(0,0)}}
\def\psCircle@ii(#1){\pscircle@do(#1){\psk@radius}}
\def\pswedge{\pst@object{pswedge}}
\def\pswedge@i{\@ifnextchar({\pswedge@ii}{\pswedge@ii(0,0)}}
\def\pswedge@ii(#1)#2#3#4{%
  \begin@ClosedObj
  \pssetlength\pst@dimc{#2}
  \pst@getangle{#3}\pst@tempa
  \pst@getangle{#4}\pst@tempb
  \pst@@getcoor{#1}%
  \def\pst@linetype{1}%
  \addto@pscode{%
    \pst@coor
    2 copy
    moveto
    \pst@number\pst@dimc \psk@dimen CLW mul sub % Adjusted radius
    \pst@tempa \pst@tempb
    arc
    closepath}%
  \showpointsfalse
  \end@ClosedObj%
}
\def\tx@Ellipse{Ellipse }
\def\psellipse{\pst@object{psellipse}}
\def\psellipse@i(#1){\@ifnextchar({\psellipse@ii(#1)}{\psellipse@ii(0,0)(#1)}}
\def\psellipse@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{%
    0 360
    \pst@coor
    \ifdim\psk@dimen\p@=\z@\else
      \psk@dimen CLW mul
      dup 4 -1 roll sub neg 3 1 roll sub
    \fi
    \pst@tempa
    \tx@Ellipse
    closepath%
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj%
}
\def\multips{\@ifnextchar({\def\pst@par{}\multips@ii}{\multips@i}}
\def\multips@i#1{\def\pst@par{rot=#1}\multips@ii}
\def\multips@ii(#1){\@ifnextchar({\multips@iii(#1)}{\multips@iii(\z@,\z@)(#1)}}
\long\def\multips@iii(#1)(#2)#3#4{%
  \begingroup
%----------------- hv 1.10 ------------------
  \pst@killglue
%----------------- hv 1.10 ------------------
  \use@par
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \pst@cnta=#3\relax
  \init@pscode
  \addto@pscode{%
    \pst@tempa T \the\pst@cnta\space \pslbrace
    gsave \ifx\psk@rot\@empty\else\psk@rot rotate \fi}%
  \hbox to\z@{%
    \def\init@pscode{%
      \addto@pscode{%
        gsave
        \pst@number\pslinewidth SLW
        \pst@usecolor\pslinecolor}}%
    \def\use@pscode{\addto@pscode{grestore}}%
    \def\psclip##1{\pst@misplaced\psclip}%
    \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
    #4%
  }%
  \addto@pscode{grestore \pst@coor T \psrbrace repeat}%
  \leavevmode
  \use@pscode
  \endgroup
  \ignorespaces}
\def\psscalebox#1{\pst@makebox{\ps@scalebox{#1}}}
\def\ps@scalebox#1{%
  \begingroup
  \pst@getscale{#1}\pst@tempa
  \let\pst@tempc\pst@tempg
  \let\pst@tempd\pst@temph
  \ps@@scalebox
  \endgroup}
\def\ps@@scalebox{%
  \leavevmode
  \hbox{%
    \ifdim\pst@tempd\p@<\z@
      \pst@dimg=\pst@tempd\ht\pst@hbox
      \pst@dimh=\pst@tempd\dp\pst@hbox
      \dp\pst@hbox=-\pst@dimg
      \ht\pst@hbox=-\pst@dimh
    \else
      \ht\pst@hbox=\pst@tempd\ht\pst@hbox
      \dp\pst@hbox=\pst@tempd\dp\pst@hbox
    \fi
    \pst@dima=\pst@tempc\wd\pst@hbox
    \ifdim\pst@dima<\z@\kern-\pst@dima\fi
    \pst@Verb{CP CP translate \pst@tempa \tx@NET}%
    \hbox to \z@{\box\pst@hbox\hss}%
    \pst@Verb{%
      CP CP translate
      1 \pst@tempc div 1 \pst@tempd div scale
      \tx@NET}%
    \ifdim\pst@dima>\z@\kern\pst@dima\fi%
  }%
}
\pslongbox{Scalebox}{\psscalebox}
%
\def\psscaleboxto(#1,#2){\pst@makebox{\ps@scaleboxto(#1,#2)}}
\def\ps@scaleboxto(#1,#2){%
  \begingroup
  \pssetlength\pst@dima{#1}%
  \pssetlength\pst@dimb{#2}%
  \ifdim\pst@dima=\z@\else
    \pst@divide{\pst@dima}{\wd\pst@hbox}\pst@tempc
    \edef\pst@tempc{\pst@tempc\space}%
  \fi
  \ifdim\pst@dimb=\z@
    \ifdim\pst@dima=\z@
      \@pstrickserr{%
        \string\psscaleboxto\space dimensions cannot both be zero}\@ehpa
      \def\pst@tempa{}%
      \def\pst@tempc{1 }%
      \def\pst@tempd{1 }% 
    \else
      \let\pst@tempd\pst@tempc
    \fi
  \else
    \pst@dimc=\ht\pst@hbox
    \advance\pst@dimc\dp\pst@hbox
    \pst@divide{\pst@dimb}{\pst@dimc}\pst@tempd
    \edef\pst@tempd{\pst@tempd\space}%
    \ifdim\pst@dima=\z@ \let\pst@tempc\pst@tempd \fi
  \fi
  \edef\pst@tempa{\pst@tempc \pst@tempd scale }%
  \ps@@scalebox
  \endgroup}
\pslongbox{Scaleboxto}{\psscaleboxto}
%
\def\tx@Rot{Rot }
\def\psrotateleft{\pst@makebox{\ps@rotateleft\pst@hbox}}
\def\ps@rotateleft#1{%
\leavevmode\hbox{\hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
\pst@Verb{90 \tx@Rot}
\vbox to \z@{\vss\hbox to \z@{\box#1\hss}\vskip\z@}%
\pst@Verb{-90 \tx@Rot}}}}
\def\psrotateright{\pst@makebox{\ps@rotateright\pst@hbox}}
\def\ps@rotateright#1{%
% ----------- hv begin 2004-05-07 ----------- patch 15
%    \hbox{%
  \leavevmode\hbox{%
% ----------- hv end 2004-05-07 ----------- patch 15
  \hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
  \pst@Verb{-90 \tx@Rot}
  \vbox to \z@{\hbox to \z@{\hss\box#1}\vss}%
  \pst@Verb{90 \tx@Rot}}}}
\def\psrotatedown{\pst@makebox{\ps@rotatedown\pst@hbox}}
\def\ps@rotatedown#1{%
\hbox{\hskip\wd#1\vbox{\vskip\ht#1\vskip\dp#1%
\pst@Verb{180 \tx@Rot}%
\vbox to \z@{\hbox to \z@{\box#1\hss}\vss}%
\pst@Verb{-180 \tx@Rot}}}}
\pslongbox{Rotateleft}{\psrotateleft}
\pslongbox{Rotateright}{\psrotateright}
\pslongbox{Rotatedown}{\psrotatedown}
% ----------- hv begin 2004-09-23 ----------- 1.11
% compatibility stuff 
\let\rotateleft\psrotateleft
\let\rotateright\psrotateright
\let\rotatedown\psrotatedown
% ----------- hv end 2005-09-23 ----------- 1.11
\def\pst@starbox{%
\setbox\pst@hbox\hbox{\psframebox*[boxsep=false]{\unhbox\pst@hbox}}}
\def\pst@@makesmall#1{%
\setbox#1=\hbox to\z@{\hss\vbox to \z@{\vss\box#1\vss}\hss}}
\def\pst@@@makesmall#1{%
\pst@dimh=\psk@xref\wd#1%
\ifx\psk@yref\relax
\pst@dimg=\dp#1%
\else
\pst@dimg=\psk@yref\ht#1%
\advance\pst@dimg\psk@yref\dp#1%
\fi
\setbox#1=\hbox to\z@{%
\kern-\pst@dimh\vbox to\z@{\vss\box#1\kern-\pst@dimg}\hss}}
\def\psset@ref#1{\pst@expandafter\psset@@ref{#1}\@empty,,\@nil}
\def\psset@@ref#1#2,#3,#4\@nil{%
  \def\psk@xref{.5}%
  \def\psk@yref{.5}%
  \let\pst@makesmall\pst@@@makesmall
  \ifx\@empty#3\@empty
    \@nameuse{getref@#1}%
    \@nameuse{getref@#2}%
  \else
    \pst@checknum{#1#2}\psk@xref
    \pst@checknum{#3}\psk@yref
  \fi}
\def\getref@c{\let\pst@makesmall\pst@@makesmall}
\def\getref@t{\def\psk@yref{1}}
\def\getref@b{\def\psk@yref{0}}
\def\getref@B{\let\psk@yref\relax}
\def\getref@l{\def\psk@xref{0}}
\def\getref@r{\def\psk@xref{1}}
\psset@ref{c}
\def\psset@rot#1{%
\pst@expandafter{\@ifnextchar*{\psset@@@rot}{\psset@@rot}}{#1}\@nil}
\def\psset@@rot#1\@nil{%
\def\next##1@#1=##2@##3\@nil{%
\ifx\relax##2%
\pst@getangle{#1}\psk@rot
\else
\def\psk@rot{##2}%
\fi}%
\expandafter\next\pst@rottable @#1=\relax @\@nil}
\def\psset@@@rot#1#2\@nil{%
\psset@@rot#2\@nil
\edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\def\pst@rotlist{mark RAngle /a ED cleartomark a neg }
\def\pst@rottable{%
@0=%
@U=%
@L=90 %
@D=180 %
@R=-90 %
@N=\pst@rotlist
@W=\pst@rotlist 90 add %
@S=\pst@rotlist 180 add %
@E=\pst@rotlist 90 sub }
\psset@rot{0}
\def\tx@RotBegin{RotBegin }
\def\tx@RotEnd{RotEnd }
\def\pst@rotate#1#2{%
  \ifx#1\@empty\else
  \setbox#2=\hbox{\pst@Verb{#1 \tx@RotBegin}\box#2\pst@Verb{\tx@RotEnd}}%
  \fi%
}
\def\psput@cartesian#1{%
  \hbox to \z@{\kern\pst@dimg{\vbox to \z@{\vss\box#1\vskip\pst@dimh}\hss}}%
}
\def\psput@special#1{%
  \hbox{%
    \pst@Verb{{ \pst@coor } \tx@PutCoor \tx@PutBegin}%
    \box#1%
    \pst@Verb{\tx@PutEnd}%
  }%
}
\def\tx@PutCoor{PutCoor }
\def\tx@PutBegin{PutBegin }
\def\tx@PutEnd{PutEnd }
\def\rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\rput@i}{\rput@ii}}}
\def\rput@i[#1]{\addto@par{ref={#1}}\rput@ii}
\def\rput@ii{\@ifnextchar({\rput@iv}{\rput@iii}}
\def\rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\rput@iv}{\rput@iv(\z@,\z@)}}
\def\rput@iv(#1){\pst@killglue\pst@makebox{\rput@v{#1}}}
\def\rput@v#1{%
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \pst@rotate\psk@rot\pst@hbox
    \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces%
}
\def\multirput{%
  \def\pst@par{}%
  \pst@ifstar{\@ifnextchar[{\multirput@i}{\multirput@ii}}%
}
\def\multirput@i[#1]{\addto@par{ref={#1}}\multirput@ii}
\def\multirput@ii{\@ifnextchar({\multirput@iv}{\multirput@iii}}
\def\multirput@iii#1{\addto@par{rot={#1}}\multirput@iv}
\def\multirput@iv(#1){%
  \@ifnextchar({\multirput@v(#1)}{\multirput@v(\z@,\z@)(#1)}%
}
\def\multirput@v(#1,#2)(#3,#4)#5{%
  \pst@makebox{\multirput@vi(#1,#2)(#3,#4){#5}}%
}
\def\multirput@vi(#1,#2)(#3,#4)#5{%
  \pst@killglue
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \pst@rotate\psk@rot\pst@hbox
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetxlength\pst@dimc{#3}%
    \pssetylength\pst@dimd{#4}%
    \pst@cntg=#5\relax
    \pst@cnth=\@ne
    \leavevmode
    \loop
      \vbox to \z@{%
        \vss
        \hbox to \z@{\kern\pst@dima\copy\pst@hbox\hss}%
        \vskip\pst@dimb%
      }%
      \ifnum\pst@cntg>\pst@cnth
        \advance\pst@dima\pst@dimc
        \advance\pst@dimb\pst@dimd
        \advance\pst@cnth\@ne
    \repeat 
    \endgroup
  \ignorespaces%
}
\newif\if@fixedradius
\def\cput{\pst@object{cput}}
\def\cput@i{\@fixedradiusfalse\cput@ii}
\def\cput@ii{\pst@killglue\@ifnextchar({\cput@iv}{\cput@iii}}
\def\cput@iii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\cput@iv}{\cput@iv(\z@,\z@)}%
}
\def\cput@iv(#1){\pst@makebox{\cput@v{#1}}}
  \def\cput@v#1{%
  \begingroup
    \use@par
    \setbox\pst@hbox=\hbox{%
      \psboxsepfalse
      \if@fixedradius\psCirclebox@ii\else\pscirclebox@ii\fi%
    }%
    \pst@@makesmall\pst@hbox
    \pst@rotate\psk@rot\pst@hbox
    \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces%
}
\def\Cput{\pst@object{Cput}}
\def\Cput@i{\@fixedradiustrue\cput@ii}
\newdimen\pslabelsep
\def\psset@labelsep#1{\pssetlength\pslabelsep{#1}}
\psset@labelsep{5pt}
\def\psset@refangle#1{\pst@expandafter\psset@@refangle{#1}\@nil}
\def\psset@@refangle#1\@nil{%
\def\next##1@#1=##2"##3@##4\@nil{%
\ifx\relax##2%
\pst@getangle{#1}\psk@refangle
\def\psk@uputref{}%
\else
\def\psk@refangle{##2 }%
\def\psk@uputref{##3}%
\fi}%
\expandafter\next\pst@refangletable @#1=\relax"@\@nil}
\def\pst@refangletable{%
@r=0"20%
@u=90"02%
@l=180"10%
@d=-90"01%
@ur=45"22%
@ul=135"12%
@dr=-135"21%
@dl=-45"11}
\psset@refangle{0}
% DG/SR modification begin - Mar. 24, 1999 - Patch 10
%\def\uput{\def\pst@par{}\@ifnextchar[{\uput@ii}{\uput@i}}
\def\uput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\uput@ii}{\uput@i}}} 
% DG/SR modification end
\def\uput@i#1{\addto@par{labelsep=#1}\uput@ii}
\def\uput@ii[#1]{%
\addto@par{refangle={#1}}%
\@ifnextchar({\uput@iv}{\uput@iii}}
\def\uput@iii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\uput@iv}{\uput@iv(\z@,\z@)}}
\def\uput@iv(#1){\pst@killglue\pst@makebox{\uput@v{#1}}}
\def\uput@v#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\uput@vi
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\uput@vi{%
\ifx\psk@uputref\@empty
\uput@vii\tx@UUput{}%
\else
\ifx\psk@rot\@empty
\expandafter\uput@viii\psk@uputref
\else
\uput@vii\tx@UUput{}%
\fi
\fi}
\def\uput@vii#1#2{%
  \edef\pst@coor{%
    \pst@number\pslabelsep
    #2%
    \pst@number{\wd\pst@hbox}%
    \pst@number{\ht\pst@hbox}%
    \pst@number{\dp\pst@hbox}%
    \psk@refangle\space \ifx\psk@rot\@empty\else\psk@rot\space sub \fi
    \tx@Uput #1}%
  \setbox\pst@hbox=\hbox to\z@{\hss\vbox to\z@{\vss\box\pst@hbox\vss}\hss}%
  \setbox\pst@hbox=\psput@special\pst@hbox
  \ifx\psk@rot\@empty\else\pst@rotate\psk@rot\pst@hbox\fi}
\def\uput@viii#1#2{%
  \ifnum#1>\z@\ifnum#2>\z@\pslabelsep=.707\pslabelsep\fi\fi
  \setbox\pst@hbox=\vbox to\z@{%
    \ifnum#2=1 \vskip\pslabelsep\else\vss\fi
    \hbox to\z@{%
      \ifnum#1=2 \hskip\pslabelsep\else\hss\fi
      \box\pst@hbox
      \ifnum#1=1 \hskip\pslabelsep\else\hss\fi}%
    \ifnum#2=2 \vskip\pslabelsep\else\vss\fi}}
\def\tx@Uput{Uput }
\def\tx@UUput{UUput }
\def\Rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Rput@ii}{\Rput@i}}}
\def\Rput@i#1{\addto@par{labelsep=#1}\Rput@ii}
\def\Rput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Rput@iv}{\Rput@iii}}
\def\Rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\Rput@iv}{\Rput@iv(\z@,\z@)}}
\def\Rput@iv(#1){\pst@killglue\pst@makebox{\Rput@v{#1}}}
\def\Rput@v#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\Rput@vi
\pst@makesmall\pst@hbox
\pst@rotate\psk@rot\pst@hbox
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\Rput@vi{%
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pslabelsep
\dp\pst@hbox=\pst@dimg
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg\pslabelsep
\ht\pst@hbox=\pst@dimg
\setbox\pst@hbox\hbox{\kern\pslabelsep\box\pst@hbox\kern\pslabelsep}}%
\def\oldpsput{%
\def\pst@par{}\pst@ifstar{\@ifnextchar[{\oldpsput@i}{\oldpsput@ii}}}
\def\oldpsput@i[#1]{\addto@par{ref={#1}}\oldpsput@ii}
\def\oldpsput@ii{\@ifnextchar<{\oldpsput@iii}{\oldpsput@iv}}
\def\oldpsput@iii<#1>{\rput@iii{#1}}
\def\OldPsput{\let\psput\oldpsput}
\def\NewPsput{\let\psput\rput}
%
% ----------- 1.10/12 beg hv -------------------
\newpsstyle{gridstyle}{subgriddiv=0,gridcolor=lightgray,griddots=10,gridlabels=8pt}
\newif\ifshowgrid
\def\psset@showgrid#1{\@nameuse{showgrid#1}}
\psset@showgrid{false}
\newdimen\psk@shift
\def\psset@shift#1{\pssetlength\pst@dimg{#1}%
  \psk@shift\pst@dimg}
%  \global\psk@shift\pst@dimg}
\psset@shift{0}
% ----------- 1.10/12 end hv -------------------
%
\def\pspicture{\begingroup\pst@ifstar\pst@picture}
\def\pst@picture{%
\@ifnextchar[{\pst@@picture}{\pst@@picture[]}}
\def\pst@@picture[#1]#2(#3,#4){%
\@ifnextchar({\pst@@@picture[#1](#3,#4)}%
{\pst@@@picture[#1](0,0)(#3,#4)}}
%
\def\pst@@@picture[#1](#2,#3)(#4,#5){%
  \pssetxlength\pst@dima{#2}%
  \pssetylength\pst@dimb{#3}%
  \pssetxlength\pst@dimc{#4}%
  \pssetylength\pst@dimd{#5}%
  \ifdim\pst@dima>\pst@dimc%
    \pst@dimg=\pst@dima%
    \pst@dima=\pst@dimc%
    \pst@dimc=\pst@dimg%
  \fi%
  \ifdim\pst@dimb>\pst@dimd%
    \pst@dimg=\pst@dimb%
    \pst@dimb=\pst@dimd%
    \pst@dimd=\pst@dimg%
  \fi%
  \setbox\pst@hbox=\hbox\bgroup%
  \begingroup\KillGlue%
  \@ifundefined{@latexerr}{}{\let\unitlength\psunit}%
  \edef\pic@coor{(#2,#3)(#2,#3)(#4,#5)}%
% ----------- 1.10/12 beg hv -------------------
  \psset{showgrid=false}%                % for nested pspicture environemnets
  \def\pst@tempA{#1}%
  \ifx\pst@tempA\@empty\else\psset{#1}\fi% sets the shift and grid option
  \ifshowgrid\psgrid[style=gridstyle]\fi%
% ----------- 1.10/12 end hv -------------------
%  \ignorespaces%
}
\def\pic@coor{(0,0)(0,0)(10,10)}
\newdimen\pst@shift
\def\endpspicture{%
  \pst@killglue
  \global\pst@shift=\psk@shift% in fact of the following endgroup
  \endgroup
  \egroup
  \ifdim\wd\pst@hbox=\z@\else
    %\@pstrickserr{Extraneous space in the pspicture environment}%
    %{Type \space <return> \space to proceed.}%
  \fi
  \ht\pst@hbox=\pst@dimd
  \dp\pst@hbox=-\pst@dimb
  \setbox\pst@hbox=\hbox{%
    \kern-\pst@dima
% ----------- 1.10/12 beg hv -------------------
%    \advance\pst@dimd-\pst@dimb%
%    \pst@dimd=\pst@shift\pst@dimd%
%    \advance\pst@dimd\pst@dimb
    \pst@dimd-\pst@shift
% ----------- 1.10/12 end hv -------------------
    \advance\pst@dimd\pst@dimb
    \lower\pst@dimd%
    \box\pst@hbox%
    \kern\pst@dimc}%
  \if@star\setbox\pst@hbox=\hbox{\clipbox@@\z@}\fi
  \leavevmode\box\pst@hbox
  \endgroup%
  \global\psk@shift\z@% restore value
}
\@namedef{pspicture*}{\pspicture*}
\@namedef{endpspicture*}{\endpspicture}
%
\def\tx@BeginOL{BeginOL }
\def\tx@InitOL{InitOL }
\def\pst@initoverlay#1{\pst@Verb{\tx@InitOL /TheOL (#1) def}}
\def\AltOverlayMode{%
  \def\pst@initoverlay##1{%
    \pst@Verb{%
      \tx@InitOL
      /Visible { initclip } def
      /Invisible {
        CP newpath OLUnit itransform moveto clip newpath moveto
      } def
      /TheOL (##1) def}}}
\def\pst@overlay#1{%
  \edef\curr@overlay{#1}%
  \pst@Verb{(#1) BOL}%
  \aftergroup\pst@endoverlay}
\def\pst@endoverlay{%
  \pst@Verb{(\curr@overlay) BOL}}
\def\curr@overlay{all}
\newbox\theoverlaybox
\def\overlaybox{%
  \global\setbox\theoverlaybox=\hbox\bgroup
  \begingroup
  \let\psoverlay\pst@overlay
  \def\overlaybox{%
    \@pstrickserr{Overlays cannot be nested}\@eha}%
  \def\putoverlaybox{%
    \@pstrickserr{You must end the overlay box
         before using \string\putoverlaybox}}%
  \psoverlay{main}%
  \ignorespaces}
\def\endoverlaybox{\endgroup\egroup}
\def\putoverlaybox#1{%
\hbox{\pst@initoverlay{#1}\copy\theoverlaybox}}
\def\psoverlay{\@pstrickserr{\string\psoverlay\space
can only be used after \string\overlaybox}}
\ifx\pstcustomize\relax \input pstricks.con \fi
\catcode`\@=\PstAtCode\relax
%
\endinput
%%
%% END: pstricks.tex

